Pushing the Boundary: Specialising Deep Configuration Performance Learning

Software systems often have numerous configuration options that can be adjusted to meet different performance requirements. However, understanding the combined impact of these options on performance is often challenging, especially with limited real-world data. To tackle this issue, deep learning techniques have gained popularity due to their ability to capture complex relationships even with limited samples. This thesis begins with a systematic literature review of deep learning techniques in configuration performance modeling, analyzing 85 primary papers out of 948 searched papers. It identifies knowledge gaps and sets three objectives for the thesis. The first knowledge gap is the lack of understanding about which encoding scheme is better and in what circumstances. To address this, the thesis conducts an empirical study comparing three popular encoding schemes. Actionable suggestions are provided to support more reliable decisions. Another knowledge gap is the sparsity inherited from the configuration landscape. To handle this, the thesis proposes a model-agnostic and sparsity-robust framework called DaL, which uses a "divide-and-learn" approach. DaL outperforms state-of-the-art approaches in accuracy improvement across various real-world systems. The thesis also addresses the limitation of predicting under static environments by proposing a sequential meta-learning framework called SeMPL. Unlike traditional meta-learning frameworks, SeMPL trains meta-environments in a specialized order, resulting in significantly improved prediction accuracy in multi-environment scenarios. Overall, the thesis identifies and addresses critical knowledge gaps in deep performance learning, significantly advancing the accuracy of performance prediction.

==> Chapter-DAL/related.tex <==
\section{Related Work}
\label{chap-dal:related}

This section discusses the related work in light of the key contributions in \Model.


\subsection{Analytical Models} 

Predicting software performance can be done by analyzing the code structure and architecture of the systems~\citep{di2004compositional,DBLP:conf/icse/VelezJSAK21}. For example,~\citet{di2004compositional} apply queuing network to model the latency of requests processed by the software.~\citet{DBLP:conf/icse/VelezJSAK21} use local measurements and
dynamic taint analysis to build a model that can predict performance for part of the configuration code. However, analytical models require full understanding and access to the software's internal states, which may not always be possible/feasible.  Further, due to the theoretical assumption or limitations of the measurement tool, analytical models are often restricted to certain performance metrics, most commonly time-related ones such as runtime and latency. \Model~is not restricted to those scenarios as it is a data-driven approach while still being designed to cater to the unique sparse nature of configuration data.


\subsection{Statistical Learning-based Models} 

Data-driven learning has relied on various statistical models, such as linear regressions~\citep{DBLP:journals/sqj/SiegmundRKKAS12,DBLP:conf/sigsoft/SiegmundGAK15,DBLP:journals/tc/SunSZZC20,DBLP:journals/is/KangKSGL20}, tree-liked model~\citep{DBLP:conf/icdcs/HsuNFM18,DBLP:conf/kbse/SarkarGSAC15,DBLP:journals/corr/abs-1801-02175}, fourier-learning models~\citep{zhang2015performance,DBLP:conf/icsm/Ha019}, and even transfer learning~\citep{DBLP:conf/sigsoft/JamshidiVKS18,DBLP:journals/tse/KrishnaNJM21,DBLP:conf/kbse/JamshidiSVKPA17}, \textit{etc}. Among others, \texttt{SPLConqueror}~\citep{DBLP:journals/sqj/SiegmundRKKAS12} utilizes linear regression
combined with different sampling methods and a step-wise feature selection to capture the interactions between configuration options. \texttt{DECART}~\citep{DBLP:journals/ese/GuoYSASVCWY18} is an improved CART with an efficient sampling method~\citep{zhang2015performance}. Jamshidi and Casale~\citep{DBLP:conf/mascots/JamshidiC16} use Gaussian Process (GP) to model configuration performance, which is also gradually updated via Bayesian Optimization. However, recent work reveals that those approaches do not work well with small datasets~\citep{DBLP:conf/icse/HaZ19}, which is rather common for configurable software systems due to their expensive measurements. This is a consequence of not fully handling the sparsity in configuration data. Further, they come with various restrictions and prerequisites, e.g., \texttt{DECART} does not work on mixed systems while \texttt{SPLConqueror} needs an extensive selection of the right sampling method(s); GP has also been proved to struggle in modeling the sparse configuration data~\citep{DBLP:journals/corr/abs-1801-02175}. 


In contrast, it is shown that \Model~produces significantly more accurate results while not limited to those restrictions. In addition, the paradigm of dividable learning underpins \Model~prevent it from suffering the particular pitfalls of a single machine learning algorithm, as it can be paired with different local models.



\subsection{Deep Learning-based Models}


A variety of studies apply deep neural networks with multiple layers to predict configuration performance~\citep{DBLP:conf/icse/HaZ19, DBLP:conf/esem/ShuS0X20,DBLP:conf/sbac-pad/NemirovskyAMNUC17,app11083706,DBLP:journals/concurrency/FalchE17,DBLP:conf/iccad/KimMMSR17,DBLP:conf/sc/MaratheAJBTKYRG17,DBLP:conf/im/JohnssonMS19,DBLP:journals/jsa/ZhangLWWZH18}. Among others, \texttt{HINNPerf} uses embedding to encodes the configuration into a latent space after which a deep neural network, combined with the hierarchical regularization, is applied to handle feature sparsity. \texttt{DeepPerf}~\citep{DBLP:conf/icse/HaZ19} is a state-of-the-art DNN model with $L_{1}$ regularization to mitigate feature sparsity for any configurable systems, and it can be more accurate than many other existing approaches. The most recently proposed \texttt{Perf-AL}~\citep{DBLP:conf/esem/ShuS0X20} relied on adversarial learning that consists of a generative network to predict the performance and a discriminator network to distinguish the predictions and the actual labels. Nevertheless, existing deep learning approaches capture only the feature sparsity while ignoring the sample sparsity, causing severe risks of overfitting even with regularization in place. 

Compared with those, it has been demonstrated that, by additionally capturing sample sparsity, \Model~is able to improve the accuracy considerably with better efficiency and acceptable overhead.


\subsection{Ensemble Models}

Similar to the paradigm of dividable learning, ensemble learning also leads to different frameworks that can be paired with different local models, some of which have already been adopted for configuration performance learning. For example,~\citet{DBLP:journals/tse/ChenB17} propose an ensemble approach, paired with feature selection for mitigating feature sparsity, to model software performance. Other ensemble learning, such as Bagging~\citep{breiman1996bagging} and Boosting~\citep{schapire2003boosting} can also be similarly applied. However, those ensemble learning approaches allow different local models to share information at one or more phases of the learning pipeline:

\begin{itemize}
    \item Local models can be trained on the same data~\citep{DBLP:journals/tse/ChenB17}; or data that has been processed sequentially~\citep{schapire2003boosting}.
    \item Local models can make predictions collectively as opposed to individually~\citep{breiman1996bagging}.
\end{itemize}

While information sharing may be useful when different models learn data with high similarity; they might not be effective in coping with highly sparse data. \Model, in contrast, produces isolated local models without sharing knowledge at all phases, including training and prediction. This has been shown to be more suitable for dealing with the sample sparsity exhibited in configuration data, preventing overfitting and memorizing largely spread data samples.




\subsection{Hybrid Models}


The analytical models can be combined with data-driven ones to form a hybrid model~\citep{DBLP:conf/wosp/HanYP21,didona2015enhancing,DBLP:conf/icse/WeberAS21}. Among others,~\citet{didona2015enhancing} use linear regression and $k$NN to learn certain components of a queuing network. Conversely,~\citet{DBLP:conf/icse/WeberAS21} propose to learn the performance of systems based on the parsed source codes from the system to the function level. 

\Model~is seen as being complementary to those hybrid models due to its flexibility in selecting the local model: when needed, the local models can be replaced with hybrid ones, making itself a hybrid variant. In case the internal structure of the system is unknown, \Model~can also work in its default as a purely data-driven approach.


==> Chapter-encoding/related_work.tex <==
% \setlength{\parskip}{0em} 

\section{Related Work}
\label{chap-encoding:related}

%Learning the performance for configurable software systems has gained momentum during the past few years. Among the others, an important engineering decision to make is how to encode the configuration as a representation when training the machine learning model is a crucial engineering decision for learning software performance.

A most widely used representation for building machine/deep learning-based software performance model is the one-hot encoding~\citep{DBLP:conf/icse/SiegmundKKABRS12,DBLP:conf/kbse/GuoCASW13,DBLP:conf/kbse/BaoLWF19}. The root motivation of such encoding is derived from the fact that a configurable system can be represented by the feature model --- a tree-liked structure that captures the variability~\citep{DBLP:conf/icse/SiegmundKKABRS12}. In a feature model, each feature can be selected or deselected, which is naturally a binary option. Note that categorical and numeric configuration options can also be captured in the feature model, as long as they can be discretized~\citep{DBLP:journals/tosem/ChenLBY18}. Following this, several approaches have been developed using machine/deep learning. Among others, \citet{DBLP:conf/kbse/GuoCASW13} use the one-hot encoding combined with the DT to predict software performance, as it fits well with the feature model. \citet{DBLP:conf/kbse/BaoLWF19} also use the same encoding, and their claim is that it can better capture the options which have no ordinal relationships.

The other, perhaps more natural, encoding scheme for learning software performance is the label encoding, which has also been followed by many studies, either with~\citep{DBLP:conf/icse/Chen19b,DBLP:journals/tse/ChenB17,DBLP:conf/icse/HaZ19} or without scaling~\citep{DBLP:journals/corr/abs-1801-02175,DBLP:conf/sigsoft/SiegmundGAK15,DBLP:conf/sigsoft/NairMSA17}. For example, \citet{DBLP:journals/tse/ChenB17} directly encode the configuration options to learn the performance model with normalization to $[0,1]$. \citet{DBLP:conf/sigsoft/SiegmundGAK15} also follows the label encoding, but the binary and numeric configuration options are treated differently in the model learned with no normalization.

However, the choice between those two encoding schemes for software performance learning often lacks systematic justification, which is the gap that this empirical study aims to bridge.

In the other domains, the importance of choosing the encoding schemes for building machine/deep learning models has been discussed. For example, \citet{9020560} compare the most common encoding schemes for predicting security events using logs. The result shows that it is considerably harmful to encode the representation without systematic justification. Similarly, \citet{DBLP:journals/bmcbi/HeP16} study the effect of two encoding schemes for genetic trait prediction. A thorough analysis of the encoding schemes has been provided, together with which could be better under what cases. However, those findings cannot be directly applied in the context of software performance learning, due to two of its properties:

\begin{itemize}


\item Sampling from the configurable systems is rather expensive~\citep{DBLP:conf/icml/ZuluagaSKP13,DBLP:journals/corr/abs-1801-02175,DBLP:conf/mascots/JamshidiC16}, thus the sample size is often relatively smaller.
\item Software configuration is often sparse, i.e., the close configurations may have rather different performance~\citep{DBLP:journals/corr/abs-1801-02175,DBLP:conf/mascots/JamshidiC16}. This is because options like \texttt{cache}, when enabled, can create significant implications to the performance, but such a change is merely represented as a one-bit difference in the model. Therefore, the distribution of the data samples can be intrinsically different from the other domains.

\end{itemize}

Most importantly, this work provides an in-depth understanding of this topic for learning software performance, together with insights and suggestions under different circumstances.




==> Chapter-survey/related.tex <==
\section{Related Work}
\label{chap-reivew:related}

There are a few related surveys in the domain of performance modeling. Among others,~\citet{DBLP:journals/pe/BalsamoPI03} conduct a review of performance prediction using Queuing Network, and~\citet{DBLP:journals/tse/BalsamoMIS04} review how performance model can be used to help software development.~\citet{DBLP:journals/sigmetrics/NambiarKBSD16} emphasize the significance of performance modeling in SE tasks and calls for further research to enhance the predictive capabilities of performance models, and~\citet{DBLP:conf/wosp/PereiraA0J20} seek to understand to what extent are sampling strategies sensitive to performance prediction of configurable systems.  A recent work~\citep{DBLP:journals/spe/HanYY23} classifies software performance learning studies into 6 categories, provides a mapping of them within these categories, and highlights potential weaknesses of the literature. Further, surveys on performance modeling for specific categories of configurable software systems exist. For example, there are reviews on the performance models for distributed systems~\citep{DBLP:conf/cisis/PllanaBB07,DBLP:journals/tpds/Lopez-NovoaMM15} and~\citet{DBLP:journals/tjs/Flores-Contreras21} survey the performance prediction methods for parallel applications published between 2005 and 2020. Similarly,~\citet{DBLP:conf/sc2/FrankHLB17} review 34 studies on performance modeling for multi-core systems, and performance learning and tuning techniques for mobile application systems are reviewed by~\citet{DBLP:journals/tse/HortKSH22}. However, the above work does not focus on how deep learning can be used in the performance model building for configurable software in general. 

On the other hand, several surveys have been conducted on the application of deep learning in software engineering. For example,~\citet{DBLP:journals/csur/YangXLG22} investigates the deep learning related techniques for software engineering tasks, including the DL models, data preprocessing methods, SE tasks, and model optimization methods, while an SLR on deep learning is also conducted by~\citet{DBLP:journals/tosem/WatsonCNMP22}, which provides a research roadmap and guidelines for future exploration in the context of software engineering.~\citet{DBLP:journals/tosem/LiuGXLGY22} investigates the reproducibility and applicability of DL studies in SE and observes that a significant number of them have overlooked this challenge. A novel work~\citep{DBLP:journals/tse/WangHGGZFSLZN23} explores the use of ML/DL techniques in various SE tasks and the challenges and differences between ML and DL. Yet, these studies do not focus on a specific SE task like performance learning, but rather provide a general review of software engineering. 

Moreover, an SLR by~\citet{DBLP:journals/jss/PereiraAMJBV21} explores the application objectives, sampling, learning and measuring methods applied, and evaluation methods related to machine learning models for performance modeling, which is the most similar to our work. However, the focus of this study is on deep learning models, which is a specific type of machine learning, and cover a wider range of techniques such as preprocessing, hyperparameter tuning, and sparsity handling methods. Besides, they did not discuss and justify the good and bad practices in the field.


In summary, this survey differs from the above on the following points:

\begin{itemize}
    \item This SLR focuses explicitly on deep learning-based performance modeling for configurable software, encompassing the latest trends observed over the past 10 years.
    \item The review covers aspects that have not been summarized before, such as the use of data preprocessing, encoding scheme, sparsity handling, hyper-parameter tuning, statistical test and effect size, dynamic environments, and public repository.
    \item The study discloses and justifies the positive and negative practices, which have not been revealed previously, with a summary of knowledge gaps to shed light on future works in the field.
\end{itemize}

==> Figures/chap-DAL/Tradeoff.tex <==

% \begin{figure}[!t]
% \centering
% \footnotesize
\begin{subfigure}{.31\columnwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{Figures/Apache_tradeoff.jpg}  
  \caption{\textsc{Apache}}
  \label{fig:tradeoff-Apache}
\end{subfigure}
\begin{subfigure}{.31\columnwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/BDBC_tradeoff.jpg} 
  \caption{\textsc{BDB-C}}
  \label{fig:tradeoff-BDBC}
\end{subfigure}
\begin{subfigure}{.33\columnwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/BDBJ_tradeoff.jpg} 
  \caption{\textsc{BDB-J}}
  \label{fig:tradeoff-BDBJ}
\end{subfigure}

\begin{subfigure}{.31\columnwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{Figures/x264_tradeoff.jpg}  
  \caption{\textsc{x264}}
  \label{fig:tradeoff-x264}
\end{subfigure}
\begin{subfigure}{.31\columnwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/hsmgp_tradeoff.jpg} 
  \caption{\textsc{HSMGP}}
  \label{fig:tradeoff-Hsmgp}
\end{subfigure}
\begin{subfigure}{.31\columnwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{Figures/hipacc_tradeoff.jpg}  
  \caption{\textsc{HIPA$^{cc}$}}
  \label{fig:tradeoff-hipacc}
\end{subfigure}


\begin{subfigure}{.31\columnwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/VP8_tradeoff.jpg} 
  \caption{\textsc{VP8}}
  \label{fig:tradeoff-VP8}
\end{subfigure}
% \hspace{5mm}
\begin{subfigure}{.31\columnwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/Irzip_tradeoff.jpg} 
  \caption{\textsc{Lrzip}}
  \label{fig:tradeoff-Lrzip}
\end{subfigure}
\hspace{4mm}
\begin{subfigure}{.15\columnwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/legend.png} 
%   \label{fig:legend}
%   \vspace{8mm}
\end{subfigure}

%     \caption{The total Scott-Knott scores for each subject system on both time and MRE. Only the Pareto-optimal models are presented.}
%     \label{fig:tradeoff}
% \end{figure}

==> Figures/chap-encoding/exp.tex <==
% CS Table for RQ2
\begin{table*}[t!]
    % \caption{Scott-Knott rank on MHPerf~(with or without comments, which are highlighted in \setlength{\fboxsep}{1.5pt}\colorbox{blue!10}{blue} and \setlength{\fboxsep}{1.5pt}\colorbox{red!10}{red}, respectively) against state-of-the-arts. The formats are the same as Table}
      \caption{Scott-Knott rankings and boxplot of RMSE of the 7 ML models with 3 encoding methods, for the 5 systems. 'OH', 'LAB' and 'SCA' stand for one-hot, label and scaled label encoding, respectively. A higher rank means the RMSE is lower and therefore the model with the encoding is better.}
    \label{tab:exp3}
  \begin{center}
    \begin{adjustbox}{max width = \textwidth}
     
\footnotesize
    \begin{tabular}{c@{}c@{}c}
        \begin{tabular}{lcccl}
            \cellcolor[gray]{1}\textbf{Classifier} & \cellcolor[gray]{1}\textbf{Rank} &     \cellcolor[gray]{1}\textbf{Med} & \cellcolor[gray]{1}\textbf{IQR} & \cellcolor[gray]{1}\\
            \hline
            % \cellcolor{blue!10}MHPerf & \cellcolor{blue!10}1 &\cellcolor{blue!10} 0.857 & \cellcolor{blue!10}0.025 & \cellcolor{blue!10} \quart{-5}{25}{85.7}{100}\\
NN\_SCA & 10 & 2944.45 & 0.39 & \quart{6.52}{0.39}{6.73}{100.00} \\
NN\_LAB & 10 & 2943.38 & 0.30 & \quart{6.57}{0.30}{6.73}{100.00} \\
NN\_OH & 10 & 2951.74 & 0.31 & \quart{6.64}{0.31}{6.75}{100.00} \\
KRR\_OH & 9 & 3014.68 & 0.19 & \quart{6.78}{0.19}{6.89}{100.00} \\
LR\_OH & 8 & 3020.36 & 0.21 & \quart{6.79}{0.21}{6.91}{100.00} \\
LR\_LAB & 8 & 3019.55 & 0.19 & \quart{6.80}{0.19}{6.91}{100.00} \\
RF\_SCA & 8 & 3019.63 & 0.20 & \quart{6.79}{0.20}{6.91}{100.00} \\
RF\_LAB & 8 & 3019.52 & 0.20 & \quart{6.79}{0.20}{6.91}{100.00} \\
KRR\_LAB & 8 & 3024.03 & 0.19 & \quart{6.81}{0.19}{6.92}{100.00} \\
LR\_SCA & 8 & 3026.49 & 0.19 & \quart{6.83}{0.19}{6.92}{100.00} \\
KRR\_SCA & 8 & 3028.21 & 0.19 & \quart{6.83}{0.19}{6.93}{100.00} \\
RF\_OH & 7 & 3060.11 & 0.20 & \quart{6.86}{0.20}{7.00}{100.00} \\
DT\_SCA & 6 & 3093.12 & 0.21 & \quart{7.00}{0.21}{7.07}{100.00} \\
DT\_LAB & 6 & 3097.61 & 0.22 & \quart{6.98}{0.22}{7.08}{100.00} \\
DT\_OH & 6 & 3095.11 & 0.25 & \quart{7.00}{0.25}{7.08}{100.00} \\
KNN\_SCA & 5 & 8968.09 & 1.54 & \quart{19.90}{1.54}{20.51}{100.00} \\
KNN\_OH & 4 & 15772.52 & 0.85 & \quart{35.78}{0.85}{36.07}{100.00} \\
KNN\_LAB & 3 & 22114.97 & 0.99 & \quart{49.96}{0.99}{50.57}{100.00} \\
SVR\_OH & 2 & 41917.30 & 5.73 & \quart{92.16}{5.73}{95.86}{100.00} \\
SVR\_SCA & 1 & 42228.88 & 5.85 & \quart{92.76}{5.85}{96.57}{100.00} \\
SVR\_LAB & 1 & 42229.54 & 5.86 & \quart{92.77}{5.86}{96.57}{100.00} \\

        \end{tabular} & 
        \begin{tabular}{|lcccl}
           \cellcolor[gray]{1}\textbf{Classifier} & \cellcolor[gray]{1}\textbf{Rank} &     \cellcolor[gray]{1}\textbf{Med} & \cellcolor[gray]{1}\textbf{IQR} & \cellcolor[gray]{1}\\
            \hline
            NN\_OH & 12 & 2497.07 & 0.10 & \quart{0.61}{0.10}{0.67}{100.00} \\
NN\_SCA & 11 & 2887.66 & 0.20 & \quart{0.72}{0.20}{0.78}{100.00} \\
NN\_LAB & 10 & 3019.11 & 0.34 & \quart{0.71}{0.34}{0.81}{100.00} \\
DT\_SCA & 9 & 15621.77 & 5.92 & \quart{2.61}{5.92}{4.19}{100.00} \\
DT\_LAB & 9 & 15621.69 & 5.92 & \quart{2.61}{5.92}{4.19}{100.00} \\
RF\_SCA & 8 & 25417.20 & 3.37 & \quart{5.50}{3.37}{6.82}{100.00} \\
RF\_LAB & 8 & 25457.00 & 3.18 & \quart{5.70}{3.18}{6.83}{100.00} \\
DT\_OH & 7 & 59610.67 & 9.35 & \quart{10.61}{9.35}{16.00}{100.00} \\
RF\_OH & 7 & 57173.71 & 5.31 & \quart{13.27}{5.31}{15.35}{100.00} \\
KNN\_LAB & 6 & 121668.37 & 3.96 & \quart{30.25}{3.96}{32.66}{100.00} \\
KNN\_SCA & 5 & 151716.91 & 3.54 & \quart{38.37}{3.54}{40.73}{100.00} \\
KNN\_OH & 4 & 168726.75 & 2.81 & \quart{43.77}{2.81}{45.30}{100.00} \\
KRR\_OH & 3 & 192199.55 & 3.73 & \quart{49.63}{3.73}{51.60}{100.00} \\
LR\_OH & 2 & 193658.25 & 3.88 & \quart{49.99}{3.88}{51.99}{100.00} \\
LR\_SCA & 2 & 194094.27 & 3.76 & \quart{50.36}{3.76}{52.11}{100.00} \\
LR\_LAB & 2 & 194648.94 & 3.79 & \quart{50.50}{3.79}{52.26}{100.00} \\
KRR\_SCA & 2 & 194588.83 & 3.84 & \quart{50.46}{3.84}{52.24}{100.00} \\
KRR\_LAB & 2 & 195128.40 & 3.88 & \quart{50.53}{3.88}{52.39}{100.00} \\
SVR\_LAB & 1 & 321782.26 & 6.84 & \quart{83.61}{6.84}{86.39}{100.00} \\
SVR\_OH & 1 & 321878.92 & 6.86 & \quart{83.64}{6.86}{86.42}{100.00} \\
SVR\_SCA & 1 & 321923.45 & 6.86 & \quart{83.65}{6.86}{86.43}{100.00} \\
        \end{tabular} &
                \begin{tabular}{lcccl}
             \cellcolor[gray]{1}\textbf{Classifier} & \cellcolor[gray]{1}\textbf{Rank} &     \cellcolor[gray]{1}\textbf{Med} & \cellcolor[gray]{1}\textbf{IQR} & \cellcolor[gray]{1}
            \\
            \hline
            NN\_SCA & 12 & 398.39 & 8.37 & \quart{17.59}{8.37}{20.93}{100.00} \\
NN\_LAB & 12 & 398.39 & 8.37 & \quart{17.59}{8.37}{20.93}{100.00} \\
NN\_OH & 11 & 645.28 & 9.91 & \quart{27.93}{9.91}{33.90}{100.00} \\
RF\_LAB & 10 & 893.39 & 9.60 & \quart{42.73}{9.60}{46.93}{100.00} \\
RF\_SCA & 10 & 896.18 & 9.25 & \quart{42.81}{9.25}{47.08}{100.00} \\
RF\_OH & 9 & 947.02 & 11.43 & \quart{46.49}{11.43}{49.75}{100.00} \\
DT\_OH & 8 & 1104.22 & 12.32 & \quart{51.41}{12.32}{58.01}{100.00} \\
DT\_LAB & 7 & 1140.59 & 17.93 & \quart{53.16}{17.93}{59.92}{100.00} \\
DT\_SCA & 7 & 1140.63 & 17.93 & \quart{53.16}{17.93}{59.92}{100.00} \\
KNN\_OH & 6 & 1302.37 & 7.61 & \quart{63.67}{7.61}{68.42}{100.00} \\
KNN\_SCA & 5 & 1359.37 & 7.14 & \quart{68.06}{7.14}{71.41}{100.00} \\
KRR\_OH & 4 & 1378.64 & 8.30 & \quart{68.47}{8.30}{72.42}{100.00} \\
KRR\_SCA & 3 & 1410.46 & 9.14 & \quart{70.32}{9.14}{74.10}{100.00} \\
KRR\_LAB & 3 & 1411.00 & 9.15 & \quart{70.34}{9.15}{74.12}{100.00} \\
LR\_LAB & 3 & 1412.19 & 9.08 & \quart{70.45}{9.08}{74.19}{100.00} \\
LR\_SCA & 3 & 1411.56 & 9.14 & \quart{70.39}{9.14}{74.15}{100.00} \\
LR\_OH & 3 & 1411.28 & 10.07 & \quart{69.94}{10.07}{74.14}{100.00} \\
KNN\_LAB & 2 & 1502.74 & 10.07 & \quart{73.73}{10.07}{78.94}{100.00} \\
SVR\_OH & 1 & 1521.08 & 11.72 & \quart{75.65}{11.72}{79.91}{100.00} \\
SVR\_SCA & 1 & 1525.33 & 11.75 & \quart{75.84}{11.75}{80.13}{100.00} \\
SVR\_LAB & 1 & 1525.57 & 11.74 & \quart{75.85}{11.74}{80.14}{100.00} \\
        \end{tabular} \\
         \textbf{(a). \texttt{MongoDB}} & \textbf{(b). \texttt{Irzip}} & \textbf{(c). \texttt{Trimesh}}
        \\
        \\


        \begin{tabular}{|lcccl|}
            \cellcolor[gray]{1}\textbf{Classifier} & \cellcolor[gray]{1}\textbf{Rank} &     \cellcolor[gray]{1}\textbf{Med} & \cellcolor[gray]{1}\textbf{IQR} & \cellcolor[gray]{1}\\
            \hline
NN\_OH & 14 & 67.62 & 0.88 & \quart{3.18}{0.88}{3.38}{100.00} \\
NN\_LAB & 13 & 86.18 & 0.61 & \quart{4.05}{0.61}{4.31}{100.00} \\
NN\_SCA & 13 & 92.37 & 1.60 & \quart{3.97}{1.60}{4.62}{100.00} \\
RF\_OH & 12 & 164.02 & 3.99 & \quart{6.76}{3.99}{8.21}{100.00} \\
RF\_LAB & 12 & 159.83 & 4.00 & \quart{6.73}{4.00}{8.00}{100.00} \\
RF\_SCA & 12 & 158.61 & 4.00 & \quart{6.63}{4.00}{7.93}{100.00} \\
DT\_SCA & 11 & 179.07 & 3.46 & \quart{8.04}{3.46}{8.96}{100.00} \\
DT\_LAB & 11 & 181.96 & 3.40 & \quart{8.20}{3.40}{9.10}{100.00} \\
DT\_OH & 11 & 182.42 & 3.42 & \quart{8.23}{3.42}{9.13}{100.00} \\
KRR\_OH & 10 & 369.58 & 0.95 & \quart{18.17}{0.95}{18.49}{100.00} \\
KNN\_SCA & 10 & 363.34 & 2.40 & \quart{17.65}{2.40}{18.18}{100.00} \\
KNN\_OH & 9 & 438.83 & 1.24 & \quart{21.43}{1.24}{21.95}{100.00} \\
KNN\_LAB & 8 & 1008.23 & 1.43 & \quart{49.62}{1.43}{50.44}{100.00} \\
KRR\_LAB & 7 & 1113.89 & 1.61 & \quart{54.82}{1.61}{55.72}{100.00} \\
SVR\_OH & 6 & 1210.97 & 1.25 & \quart{59.93}{1.25}{60.58}{100.00} \\
KRR\_SCA & 5 & 1306.24 & 1.56 & \quart{64.59}{1.56}{65.34}{100.00} \\
SVR\_LAB & 4 & 1495.85 & 1.82 & \quart{74.05}{1.82}{74.83}{100.00} \\
SVR\_SCA & 3 & 1507.12 & 1.92 & \quart{74.76}{1.92}{75.39}{100.00} \\
LR\_SCA & 2 & 4562.24 & 1.97 & \quart{90.10}{1.97}{92.82}{100.00} \\
LR\_LAB & 2 & 4483.84 & 2.12 & \quart{90.72}{2.12}{92.45}{100.00} \\
LR\_OH & 1 & 7814.81 & 99 & \quart{90.70}{9}{99.11}{100.00} \\


        \end{tabular} &
        \begin{tabular}{lcccl}
              \cellcolor[gray]{1}\textbf{Classifier} & \cellcolor[gray]{1}\textbf{Rank} &     \hphantom{\cellcolor[gray]{1}\textbf{Med}} & \hphantom{\cellcolor[gray]{1}\textbf{IQR}} & \hphantom{\cellcolor[gray]{1}}\\
            \hline
RF\_LAB & 19 & 581.18 & 6.07 & \quart{27.64}{6.07}{29.07}{100.00} \\
NN\_OH & 19 & 446.49 & 7.94 & \quart{19.60}{7.94}{22.34}{100.00} \\
NN\_LAB & 18 & 481.45 & 6.97 & \quart{20.77}{6.97}{24.08}{100.00} \\
NN\_SCA & 17 & 671.84 & 5.32 & \quart{31.75}{5.32}{33.61}{100.00} \\
RF\_OH & 17 & 665.35 & 6.60 & \quart{30.65}{6.60}{33.28}{100.00} \\
KNN\_OH & 16 & 1021.07 & 4.49 & \quart{48.97}{4.49}{51.08}{100.00} \\
RF\_SCA & 15 & 735.36 & 4.61 & \quart{35.10}{4.61}{36.79}{100.00} \\
DT\_LAB & 14 & 739.20 & 6.96 & \quart{34.49}{6.96}{36.98}{100.00} \\
KRR\_OH & 13 & 910.47 & 4.64 & \quart{43.52}{4.64}{45.55}{100.00} \\
DT\_OH & 12 & 803.96 & 8.26 & \quart{36.70}{8.26}{40.22}{100.00} \\
DT\_SCA & 11 & 950.32 & 6.04 & \quart{45.36}{6.04}{47.54}{100.00} \\
LR\_LAB & 10 & 1046.27 & 3.38 & \quart{50.07}{3.38}{52.34}{100.00} \\
KNN\_SCA & 9 & 939.14 & 3.79 & \quart{45.49}{3.79}{46.98}{100.00} \\
LR\_SCA & 8 & 1084.04 & 3.01 & \quart{53.02}{3.01}{54.23}{100.00} \\
KRR\_LAB & 7 & 1110.85 & 3.61 & \quart{53.77}{3.61}{55.57}{100.00} \\
KRR\_SCA & 6 & 1183.43 & 3.39 & \quart{57.17}{3.39}{59.20}{100.00} \\
KNN\_LAB & 5 & 1455.11 & 4.34 & \quart{70.68}{4.34}{72.79}{100.00} \\
SVR\_LAB & 4 & 1487.67 & 4.93 & \quart{72.13}{4.93}{74.42}{100.00} \\
SVR\_OH & 3 & 1566.62 & 5.47 & \quart{76.28}{5.47}{78.37}{100.00} \\
SVR\_SCA & 2 & 1714.36 & 5.89 & \quart{83.50}{5.89}{85.76}{100.00} \\
LR\_OH & 1 & 9999.99 & 17.91 & \quart{90}{17}{99}{100.00} \\

        \end{tabular}\\
      \textbf{(d). \texttt{ExaStencils}}  & \textbf{(e). \texttt{X264-DB}}\\
    \end{tabular}
  \end{adjustbox}
   \end{center}
\end{table*}

==> Tables/chap-DAL/data_example.tex <==
% \begin{table}[]
% \centering
% \small
% \caption{An example of performance dataset. $\overline{x}$ are the configurations and $\varmathbb{P}$ is the performance value.}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
$x_{1}$ & $x_{2}$ & $x_{3}$ & $\cdots$ & $x_{n-2}$ & $x_{n-1}$ & $x_{n}$ & $\varmathbb{P}$ \\ \hline
0 & 0 & 0 & $\cdots$ & 0 & 3 & 10 & 1200 \\ 
0 & 1 & 0 & $\cdots$ & 0 & 2 & 11 & 2100 \\ 
$\cdots$        & $\cdots$  & $\cdots$       & $\cdots$       & $\cdots$       & $\cdots$ & $\cdots$ & $\cdots$ \\ 
0 & 0 & 1 & $\cdots$ & 0 & 9 & 23 & 1260 \\ 
0 & 0 & 1 & $\cdots$ & 1 & 8 & 65 & 1140 \\ \hline
\end{tabular}
% \label{tb:data_example}
% \end{table}

==> Tables/chap-DAL/vs-STOA.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[]
% \footnotesize
% \renewcommand\arraystretch{1.3}
\begin{tabular}{llllllllll}
\toprule
&
  Model &
  \textsc{Apache} &
  \textsc{BDB-C} &
  \textsc{BDB-J} &
  \textsc{x264} &
  \textsc{HSMGP} &
  \textsc{HIPA$^{cc}$} &
  \textsc{VP8} &
  \textsc{Lrzip} \\ \hline
 &
  \texttt{DeepPerf} &
  20.19(6.34) &
  75.98(70.55) &
  2.98(3.34) &
  8.39(4.77) &
  7.09(3.04) &
  9.70(1.28) &
  4.68(3.27) &
  35.40(16.59) \\
 &
  \texttt{\texttt{DECART}} &
  19.44(6.48) &
  \textbf{51.88(45.91)} &
  \textbf{2.36(0.75)} &
  9.27(2.11) &
  - &
  - &
  - &
  - \\
 &
  \texttt{Perf-AL} &
  33.57(11.34) &
  82.38(57.27) &
  37.45(2.45) &
  37.00(9.43) &
  66.70(1294.05) &
  31.99(0.06) &
  60.05(2.03) &
  58.45(0.12) \\
 &
  \texttt{\texttt{SPLConqueror} } &
  \textbf{14.44(0)} &
  86.85(0) &
  12.29(0) &
  \textbf{7.01(0)} &
  15.04(0) &
  16.68(0) &
  \textbf{29.39(0)} &
  123.7(0) \\
\multirow{-5}{*}{Size 1} &
  \Model &
  21.02(6.64) &
  74.26(67.75) &
  3.14(2.90) &
  8.23(3.05) &
  \cellcolor{green!10}\textbf{4.66(1.32)} &
  \cellcolor{green!10}\textbf{9.07(1.18)} &
  \cellcolor{green!10}\textbf{1.59(0.36)} &
  \cellcolor{green!10}\textbf{26.40(6.94)} \\ \hline
 &
  \texttt{DeepPerf} &
  9.79(4.56) &
  17.58(8.01) &
  1.91(0.68) &
  3.17(1.00) &
  3.69(0.61) &
  6.89(1.44) &
  2.39(1.21) &
  21.46(4.53) \\
 &
  \texttt{\texttt{DECART}} &
  \textbf{9.77(5.36)} &
  \textbf{13.37(7.25)} &
  \textbf{1.84(0.17)} &
  6.29(1.72) &
  - &
  - &
  - &
  - \\
 &
  \texttt{Perf-AL} &
  32.97(6.24) &
  73.99(22.51) &
  37.90(1.67) &
  34.98(7.81) &
  66.67(0.11) &
  31.98(0.06) &
  60.04(0.24) &
  58.46(0.18) \\
 &
  \texttt{\texttt{SPLConqueror} } &
  13.88(0) &
  162.91(0) &
  24.85(0) &
  6.63(0) &
  22.63(0) &
  16.96(0) &
  35.34(0) &
  171.85(0) \\
\multirow{-5}{*}{Size 2} &
  \Model &
  9.82(5.39) &
  18.32(17.04) &
  1.90(0.37) &
  \cellcolor{green!10}\textbf{3.21(1.95)} &
  \cellcolor{green!10}\textbf{2.66(0.68)} &
  \cellcolor{green!10}\textbf{5.55(0.60)} &
  \cellcolor{green!10}\textbf{1.21(0.09)} &
  \cellcolor{green!10}\textbf{15.37(6.04)} \\ \hline
 &
  \texttt{DeepPerf} &
  7.98(1.91) &
  12.47(4.08) &
  2.01(1.10) &
  2.23(0.90) &
  2.28(0.37) &
  4.68(0.90) &
  1.93(0.72) &
  18.68(3.20) \\
 &
  \texttt{\texttt{DECART}} &
  8.07(1.05) &
  7.56(5.07) &
  1.64(0.24) &
  4.57(1.03) &
  - &
  - &
  - &
  - \\
 &
  \texttt{Perf-AL} &
  31.73(4.66) &
  69.74(4.33) &
  37.19(1.70) &
  36.25(7.73) &
  66.63(0.18) &
  31.99(0.06) &
  60.02(0.29) &
  58.44(0.21) \\
 &
  \texttt{\texttt{SPLConqueror} } &
  13.99(0) &
  193.89(0) &
  25.88(0) &
  6.31(0) &
  32.46(0) &
  17.18(0) &
  36.26(0) &
  177.61(0) \\
\multirow{-5}{*}{Size 3} &
  \Model &
  \cellcolor{green!10}\textbf{7.17(2.67)} &
  \cellcolor{green!10}\textbf{5.74(6.84)} &
  \cellcolor{green!10}\textbf{1.61(0.31)} &
  \cellcolor{green!10}\textbf{1.66(0.57)} &
  \cellcolor{green!10}\textbf{1.56(0.20)} &
  \cellcolor{green!10}\textbf{4.39(0.41)} &
  \cellcolor{green!10}\textbf{1.12(0.08)} &
  \cellcolor{green!10}\textbf{11.83(4.53)} \\ \hline
 &
  \texttt{DeepPerf} &
  6.85(1.60) &
  9.06(9.76) &
  1.70(0.37) &
  1.74(0.98) &
  2.23(0.39) &
  3.58(1.00) &
  1.54(0.40) &
  15.55(1.71) \\
 &
  \texttt{\texttt{DECART}} &
  7.47(0.72) &
  5.17(5.07) &
  \textbf{1.47(0.12)} &
  3.66(1.42) &
  - &
  - &
  - &
  - \\
 &
  \texttt{Perf-AL} &
  30.67(6.84) &
  69.50(2.49) &
  37.74(2.59) &
  36.41(6.47) &
  66.63(0.14) &
  31.98(0.06) &
  59.99(0.27) &
  58.48(0.21) \\
 &
  \texttt{\texttt{SPLConqueror} } &
  13.84(0) &
  231.68(0) &
  29.01(0) &
  6.32(0) &
  33.73(0) &
  17.42(0) &
  37.14(0) &
  236.48(0) \\
\multirow{-5}{*}{Size 4} &
  \Model &
  \cellcolor{green!10}\textbf{6.59(1.77)} &
  \cellcolor{green!10}\textbf{3.68(2.78)} &
  1.61(0.29) &
  \cellcolor{green!10}\textbf{1.13(0.63)} &
  \cellcolor{green!10}\textbf{1.49(0.15)} &
  \cellcolor{green!10}\textbf{3.22(0.35)} &
  \cellcolor{green!10}\textbf{1.10(0.06)} &
  \cellcolor{green!10}\textbf{10.10(3.23)} \\ \hline
 &
  \texttt{DeepPerf} &
  6.66(1.61) &
  7.08(8.03) &
  1.69(0.48) &
  1.44(0.90) &
  1.94(0.68) &
  2.82(0.57) &
  1.45(0.23) &
  10.17(0.91) \\
 &
  \texttt{\texttt{DECART}} &
  7.14(0.89) &
  3.54(1.92) &
  \textbf{1.37(0.26)} &
  2.15(1.05) &
  - &
  - &
  - &
  - \\
 &
  \texttt{Perf-AL} &
  30.45(4.91) &
  69.29(0.69) &
  35.76(4.47) &
  36.20(3.75) &
  66.59(0.20) &
  31.97(0.14) &
  59.95(0.68) &
  58.39(0.21) \\
 &
  \texttt{\texttt{SPLConqueror} } &
  14.06(0) &
  296.68(0) &
  29.87(0) &
  6.36(0) &
  35.86(0) &
  17.69(0) &
  36.21(0) &
  208.08(0) \\
\multirow{-5}{*}{Size 5} &
  \Model &
  \cellcolor{green!10}\textbf{5.96(2.07)} &
  \cellcolor{green!10}\textbf{2.15(1.52)} &
  1.46(0.26) &
  \cellcolor{green!10}\textbf{0.79(0.33)} &
  \cellcolor{green!10}\textbf{1.16(0.08)} &
  \cellcolor{green!10}\textbf{2.39(0.22)} &
  \cellcolor{green!10}\textbf{1.07(0.05)} &
  \cellcolor{green!10}\textbf{6.60(1.34)} \\
\bottomrule
\end{tabular}
% \end{table*}


==> Tables/chap-DAL/vsDeepPerf.tex <==
% \begin{table*}[]
% \footnotesize
% \renewcommand\arraystretch{1.5}
% \caption{The median (IQR) of DeepPerf and \Model for all the subject sysmtems. 
% The \colorbox{red!10}{\textbf{cells}} mean DeepPerf is significantly better, and the \colorbox{green!10}{\textbf{cells}} mean \Model is significantly better.}
\resizebox{\textwidth}{!}{ % resize the table
\begin{tabular}{p{0.75cm}llp{0.2cm}llp{0.2cm}llp{0.2cm}llp{0.2cm}llp{0.2cm}}
\toprule
\multirow{2}{}{Subject system} &
  \multicolumn{3}{c}{Size 1} &
  \multicolumn{3}{c}{Size 2} &
  \multicolumn{3}{c}{Size 3} &
  \multicolumn{3}{c}{Size 4} &
  \multicolumn{3}{c}{Size 5} \\ \cline{2-16} 
 &
  \multicolumn{1}{l}{DeepPerf} &
  \multicolumn{1}{l}{\Model} &
  $\hat{A}_{12}$ &
  \multicolumn{1}{l}{DeepPerf} &
  \multicolumn{1}{l}{\Model} &
  $\hat{A}_{12}$ &
  \multicolumn{1}{l}{DeepPerf} &
  \multicolumn{1}{l}{\Model} &
  $\hat{A}_{12}$ &
  \multicolumn{1}{l}{DeepPerf} &
  \multicolumn{1}{l}{\Model} &
  $\hat{A}_{12}$ &
  \multicolumn{1}{l}{DeepPerf} &
  \multicolumn{1}{l}{\Model} &
  $\hat{A}_{12}$ \\ \hline
\textsc{Apache} &
  \multicolumn{1}{l}{20.19(6.34)} &
  \multicolumn{1}{l}{21.02(6.64)} &
  N &
  \multicolumn{1}{l}{9.79(4.56)} &
  \multicolumn{1}{l}{9.82(5.39)} &
  S &
  \multicolumn{1}{l}{7.98(1.91)} &
  \multicolumn{1}{l}{7.17(2.67)} &
  S &
  \multicolumn{1}{l}{6.85(1.60)} &
  \multicolumn{1}{l}{6.59(1.77)} &
  N &
  \multicolumn{1}{l}{6.66(1.61)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{5.96(2.07)}} &
  \cellcolor{green!10}\textbf{M$^\dagger$} \\ \hline
\textsc{BDB-C} &
  \multicolumn{1}{l}{75.98(70.55)} &
  \multicolumn{1}{l}{74.26(67.75)} &
  N &
  \multicolumn{1}{l}{17.58(8.01)} &
  \multicolumn{1}{l}{18.32(17.04)} &
  N &
  \multicolumn{1}{l}{12.47(4.08)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{5.74(6.84)}} &
  \cellcolor{green!10}\textbf{M$^\dagger$} &
  \multicolumn{1}{l}{9.06(9.76)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{3.68(2.78)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} &
  \multicolumn{1}{l}{7.08(8.03)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{2.15(1.52)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} \\ \hline
\textsc{BDB-J} &
  \multicolumn{1}{l}{2.98(3.34)} &
  \multicolumn{1}{l}{3.14(2.90)} &
  N &
  \multicolumn{1}{l}{1.91(0.68)} &
  \multicolumn{1}{l}{1.90(0.37)} &
  N &
  \multicolumn{1}{l}{2.01(1.10)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{1.61(0.31)}} &
  \cellcolor{green!10}\textbf{M$^\dagger$} &
  \multicolumn{1}{l}{1.70(0.37)} &
  \multicolumn{1}{l}{1.61(0.29)} &
  S &
  \multicolumn{1}{l}{1.69(0.48)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{1.46(0.26)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} \\ \hline
\textsc{x264} &
  \multicolumn{1}{l}{8.39(4.77)} &
  \multicolumn{1}{l}{8.23(3.05)} &
  N &
  \multicolumn{1}{l}{3.17(1.00)} &
  \multicolumn{1}{l}{3.21(1.95)} &
  N &
  \multicolumn{1}{l}{2.23(0.90)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{1.66(0.57)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} &
  \multicolumn{1}{l}{1.74(0.98)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{1.13(0.63)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} &
  \multicolumn{1}{l}{1.44(0.90)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{0.79(0.33)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} \\ \hline
\textsc{HSMGP} &
  \multicolumn{1}{l}{7.09(3.04)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{4.66(1.32)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} &
  \multicolumn{1}{l}{3.69(0.61)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{2.66(0.68)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} &
  \multicolumn{1}{l}{2.28(0.37)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{1.56(0.20)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} &
  \multicolumn{1}{l}{2.23(0.39)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{1.49(0.15)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
   \\ \hline
\textsc{HIPA$^{cc}$} &
  \multicolumn{1}{l}{9.70(1.28)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{9.07(1.18)}} &
  \cellcolor{green!10}\textbf{S$^\dagger$} &
  \multicolumn{1}{l}{6.89(1.44)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{5.55(0.60)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} &
  \multicolumn{1}{l}{4.68(0.90)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{4.39(0.41)}} &
  \cellcolor{green!10}\textbf{M$^\dagger$} &
  \multicolumn{1}{l}{3.58(1.00)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{3.22(0.35)}} &
  \cellcolor{green!10}\textbf{M$^\dagger$} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
   \\ \hline
\textsc{VP8} &
  \multicolumn{1}{l}{31.93(23.25)} &
  \multicolumn{1}{l}{29.73(20.29)} &
  N &
  \multicolumn{1}{l}{13.08(10.99)} &
  \multicolumn{1}{l}{9.70(11.92)} &
  S &
  \multicolumn{1}{l}{10.00(5.25)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{5.43(3.36)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} &
  \multicolumn{1}{l}{4.44(1.08)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{3.78(1.83)}} &
  \cellcolor{green!10}\textbf{M$^\dagger$} &
  \multicolumn{1}{l}{6.28(4.91)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{2.80(1.20)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} \\ \hline
\textsc{Lrzip} &
  \multicolumn{1}{l}{770.98(841.54)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{71.09(16.18)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} &
  \multicolumn{1}{l}{127.86(94.46)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{76.24(27.57)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} &
  \multicolumn{1}{l}{116.85(101)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{73.37(28.9)}} &
  \cellcolor{green!10}\textbf{L$^\dagger$} &
  \multicolumn{1}{l}{70.76(64.05)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{54.66(24.5)}} &
  \cellcolor{green!10}\textbf{M$^\dagger$} &
  \multicolumn{1}{l}{56.16(21.10)} &
  \multicolumn{1}{l}{\cellcolor{green!10}\textbf{45.13(20.0)}} &
  \cellcolor{green!10}\textbf{M$^\dagger$} \\ \bottomrule
\end{tabular}
}
% \label{tb:vsDeepperf}
% \end{table*}



==> Tables/chap-encoding/key-options.tex <==
\begin{table}[!t]
\caption{The key configuration options identified.}
\label{tb:keyopt}
\centering
%\setlength{\tabcolsep}{1.1mm}
%\scriptsize
\footnotesize
%\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{ccc|cc}
\toprule
    \textbf{System}&
    $\lvert \mathbfcal{P} \rvert$&
    \textbf{Key Option(s)}&
    $\lvert \mathbfcal{P} \rvert$&
    \textbf{Key Option(s)}\\
    \midrule
    






\textsc{Storm/WC-Azure}&
P1&
\texttt{spout\_wait}&
P2&
\texttt{spout\_wait}\\


\rowcolor{blue!10}\textsc{Storm/WC-ON-3}&
P1&
\texttt{spout\_wait}&
P2&
\texttt{spout\_wait}\\

\textsc{Storm/2WC-EC2}&
P1&
\texttt{max\_spout}, \texttt{spliter}&
P2&
\texttt{max\_spout}\\


\rowcolor{blue!10}\textsc{Storm/WC-RS-EC2}&
P1&
\texttt{max\_spout}&
P2&
\texttt{max\_spout}\\


\textsc{Storm/WC-ON-5}&
P1&
\texttt{spout}&
P2&
\texttt{count}\\


\rowcolor{blue!10}\textsc{Sort-256}&
P1&
\texttt{sort\_a}, \texttt{sort\_b}&
P2&
\texttt{sort\_a}\\


\textsc{non-CM-log}&
P1&
\texttt{multiplier}&
P2&
\texttt{multiplier}\\






    
     
   \bottomrule
   
   %\quart{of 0}{16}{10}{20}
    %\rowcolor{blue!10}\textbf{5} & \textbf{D1} & \textbf{0.80} & \textbf{0.14} & \quart{71}{14}{80}{100}\\
\end{tabular}
\centering
 \begin{tablenotes}
    \footnotesize
    \item $\lvert \mathbfcal{P} \rvert$ denotes the performance attribute.
    \end{tablenotes}
\end{table}

==> Tables/chap-encoding/pareto.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[!t]
\caption{The pareto-optimal points considering the the Scott-Knott rankings of both RMSE and training time. The \colorbox{green!40}{green cells} represent the pareto-optimal cases, i.e., no other case for the same system is better than them in both accuracy and time.}
\label{tb:rq3-pareto}
\centering
\setlength{\tabcolsep}{0.5mm}
\begin{tabular}{@{}l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c@{}}
\toprule
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}DT} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}KNN} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}KRR} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}LR} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}NN} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}RF} &
  \multicolumn{3}{c}{\cellcolor[HTML]{FFFFFF}SVR} \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}} & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA \\
\rowcolor[HTML]{EFEFEF} 
MongoDB &
   &
   &
   &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
   &
   &
   &
   &
   &
   \\
   \hline
\rowcolor[HTML]{C0C0C0} 
Irzip &
   &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
   &
  \cellcolor[HTML]{9AFF99} &
   &
   &
   &
   &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
   &
  \cellcolor[HTML]{9AFF99} &
   &
   &
   &
   &
   &
   \\
\rowcolor[HTML]{EFEFEF} 
   \hline
Trimesh &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
   &
   &
  \cellcolor[HTML]{9AFF99} &
   &
   &
   &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
   &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
   &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
   &
   &
   \\
\rowcolor[HTML]{C0C0C0} 
   \hline
ExaStencils &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
   &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
   &
   &
   &
   &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
   &
   &
   &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
   &
   &
   \\
\rowcolor[HTML]{EFEFEF} 
   \hline
X264-DB &
   &
  \cellcolor[HTML]{9AFF99} &
   &
  \cellcolor[HTML]{9AFF99} &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{9AFF99} &
   &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
   &
  \cellcolor[HTML]{9AFF99} &
   &
   &
   &
   \\ \bottomrule
\end{tabular}
\end{table*}

==> Tables/chap-encoding/rq1.tex <==
\begin{table*}[!t]
\caption{The median difference (IQR) on RMSE over 50 runs; \colorbox{blue!10}{blue cell} denotes the label encoding wins while \colorbox{red!10}{red cell} denotes the label encoding loses; white cell means a tie. N, S, M, and L denotes negligible, small, medium, and large effect size, respectively. $^\dagger$ means the comparison has a $p<0.05$. Statistically significant comparison with non-trivial effect size is shown in bold.}
\label{tb:rq1}
\centering
\setlength{\tabcolsep}{0.5mm}
%\scriptsize
\footnotesize
%\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{ccll|ll|ll|ll|ll|ll}
\toprule
    &&\multicolumn{2}{c}{\textbf{RF}} & \multicolumn{2}{c}{\textbf{$k$NN}} & \multicolumn{2}{c}{\textbf{SVR}} & \multicolumn{2}{c}{\textbf{DT}} & \multicolumn{2}{c}{\textbf{LR}} & \multicolumn{2}{c}{\textbf{KRR}}  \\
    \midrule
    
%    wc-c1-3d (SS-A)
%    wc-3c-3d (SS-C)
%    wc+wc-c4-3d (SS-D)
%    wc+rs-c4-3d (SS-F)
%    wc-5d-c5 (SS-I)
%    sort-256 (SS-B)
%    noc-CM-log (SS-H)

    
\multirow{2}{*}{\textsc{Storm/WC-Azure}}&P1&   

\cellcolor{blue!10}$-$0.90 (1.50) & \cellcolor{blue!10}N$^\dagger$
    &  \cellcolor{blue!10}{41.83 (48.18)}&\cellcolor{blue!10}{N$^\dagger$}
    &  both timeout&
    &  \cellcolor{red!10}$-$1.33 (2.34)&\cellcolor{red!10}N$^\dagger$
    &  \textbf{\cellcolor{red!10}$-$124.96 (65.42)}&\textbf{\cellcolor{red!10}S$^\dagger$}
    &  \cellcolor{blue!10}$-$73.50 (65.83) & \cellcolor{blue!10}N$^\dagger$\\
&P2&   
\cellcolor{red!10}{$-$0.94 (150.76)} & \cellcolor{red!10}{N}
    &  \cellcolor{blue!10}{9.80 (439.25)} & \cellcolor{blue!10}{N}
    &  \cellcolor{red!10}label timeout&\cellcolor{red!10}
    &  \cellcolor{blue!10}{9.92 (353.24)} & \cellcolor{blue!10}{N}
    &  \textbf{\cellcolor{blue!10}{347.84 (220.10)}} & \textbf{\cellcolor{blue!10}{M$^\dagger$}}
    &  \textbf{\cellcolor{red!10}{$-$739.91 (259.21)}} & \textbf{\cellcolor{red!10}{L$^\dagger$}}\\
\hline

\multirow{2}{*}{\textsc{Storm/WC-ON-3}}
&P1&
\textbf{\cellcolor{blue!10}{172.44 (180.15)}}&\textbf{\cellcolor{blue!10}{L$^\dagger$}}
    & \cellcolor{blue!10}{449.19 (374.46)}&\cellcolor{blue!10}{N$^\dagger$}
    &  \cellcolor{red!10}label timeout&\cellcolor{red!10}
    &  \cellcolor{blue!10}{83.24 (178.90)}&\cellcolor{blue!10}{N$^\dagger$}
    &  \textbf{\cellcolor{red!10}{$-$1368.73 (614.68)}} & \textbf{\cellcolor{red!10}{M$^\dagger$}}
    &  \textbf{\cellcolor{red!10}{$-$1003.54 (720.35)}} & \textbf{\cellcolor{red!10}{S$^\dagger$}}\\
&P2&
\textbf{\cellcolor{blue!10}{1129.18 (519.65)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{1283.71 (512.30)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \cellcolor{red!10}label timeout&\cellcolor{red!10}
    &  \textbf{\cellcolor{blue!10}{1438.48 (961.74)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{635.07 (307.12)}}&\textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{red!10}{$-$1407.99 (354.30)}}&\textbf{\cellcolor{red!10}{L$^\dagger$}}\\
\hline
    
\multirow{2}{*}{\textsc{Storm/2WC-EC2}}
&P1&   
\textbf{\cellcolor{blue!10}{2870.99 (4862.44)}} & \textbf{\cellcolor{blue!10}{S$^\dagger$}}
    &  \cellcolor{blue!10}{1726.53 (3177.50)} & \cellcolor{blue!10}{N$^\dagger$}
    &  \cellcolor{red!10}label timeout&\cellcolor{red!10}
    &  \textbf{\cellcolor{blue!10}{2037.28 (6914.90)}} & \textbf{\cellcolor{blue!10}{S$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{7896.56 (10418.86)}} & \textbf{\cellcolor{blue!10}{M$^\dagger$}}
    &  \cellcolor{blue!10}{1009.15 (2757.00)} & \cellcolor{blue!10}{N$^\dagger$}\\
&P2&   
\textbf{\cellcolor{blue!10}{409.65 (1985.19)}} & \textbf{\cellcolor{blue!10}{S$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{2363.43 (1986.66)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \cellcolor{red!10}label timeout&\cellcolor{red!10}
    &  \cellcolor{blue!10}{235.80 (2662.56)} & \cellcolor{blue!10}{N}
    &  \textbf{\cellcolor{blue!10}{4769.91 (7236.36)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{5990.96 (3483.08)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}\\
\hline

\multirow{2}{*}{\textsc{Storm/WC-RS-EC2}}
&P1&   
\textbf{\cellcolor{blue!10}{1481.49 (6532.88)}} & \textbf{\cellcolor{blue!10}{S$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{2529.33 (3890.78)}} & \textbf{\cellcolor{blue!10}{S$^\dagger$}}
    &  \cellcolor{blue!10}{113.87 (269.64)} & \cellcolor{blue!10}{N$^\dagger$}
    &  \textbf{\cellcolor{blue!10}{2158.02 (9754.71)}} & \textbf{\cellcolor{blue!10}{S$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{9764.45 (15211.68)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{1366.91 (4113.91)}} & \textbf{\cellcolor{blue!10}{S$^\dagger$}}\\
&P2&   
\cellcolor{blue!10}{417.70 (1793.86)} & \cellcolor{blue!10}{N}
    &  \textbf{\cellcolor{blue!10}{1965.56 (2704.00)}} & \textbf{\cellcolor{blue!10}{M$^\dagger$}}
    &  \textbf{\cellcolor{red!10}{$-$6668.69 (10334.43)}} & \textbf{\cellcolor{red!10}{L$^\dagger$}}
    &  \cellcolor{blue!10}{480.83 (2436.13)} & \cellcolor{blue!10}{N}
    &  \textbf{\cellcolor{blue!10}{3463.33 (8614.26)}} & \textbf{\cellcolor{blue!10}{M$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{6087.9 (3206.82)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}\\
\hline
    
\multirow{2}{*}{\textsc{STROM/WC-ON-5}}
&P1&   
\textbf{\cellcolor{blue!10}{2.54 (4.25)}} & \textbf{\cellcolor{blue!10}{S$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{7.19 (5.11)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  both timeout&
    &  \cellcolor{blue!10}{0.02 (6.20)} & \cellcolor{blue!10}{N}
    &  \textbf{\cellcolor{blue!10}{2.59 (4.45)}} & \textbf{\cellcolor{blue!10}{S$^\dagger$}}
    &  \textbf{\cellcolor{red!10}{$-$10.35 (6.40)}} & \textbf{\cellcolor{red!10}{L$^\dagger$}}\\
&P2&   
\cellcolor{blue!10}{4.60 (258.34)} & \cellcolor{blue!10}{N}
    &  \textbf{\cellcolor{blue!10}{441.00 (164.80)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{682.53 (363.20)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{red!10}{$-$117.27 (186.78)}} & \textbf{\cellcolor{red!10}{S$^\dagger$}}
    &  \textbf{\cellcolor{red!10}{$-$1277.94 (342.23)}} & \textbf{\cellcolor{red!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{red!10}{$-$2163.45 (791.86)}} & \textbf{\cellcolor{red!10}{L$^\dagger$}}\\
\hline

\multirow{2}{*}{\textsc{Sort-256}}
&P1&   
\textbf{\cellcolor{blue!10}{0.88 (0.37)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{0.92 (0.35)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \cellcolor{red!10}label timeout&\cellcolor{red!10}
    &  \textbf{\cellcolor{blue!10}{0.94 (0.60)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{0.54 (0.38)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{1.88 (1.02)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}\\
&P2&   
\textbf{\cellcolor{blue!10}{0.68 (0.25)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{0.84 (0.44)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \cellcolor{red!10}label timeout&\cellcolor{red!10}
    &  \textbf{\cellcolor{blue!10}{0.76 (0.38)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{0.62 (0.44)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{1.99 (1.02)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}\\
\hline
    
\multirow{2}{*}{\textsc{noc-CM-log}}
&P1&   
\textbf{\cellcolor{blue!10}{0.17 (0.18)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{0.49 (0.17)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \cellcolor{red!10}label timeout&\cellcolor{red!10}
    &  \textbf{\cellcolor{blue!10}{0.09 (0.17)}}& \textbf{\cellcolor{blue!10}{S$^\dagger$}}
    &  \textbf{\cellcolor{red!10}{$-$0.06 (0.15)}} & \textbf{\cellcolor{red!10}{M$^\dagger$}}
    &  \textbf{\cellcolor{red!10}{$-$1.94 (0.47)}} & \textbf{\cellcolor{red!10}{L$^\dagger$}}\\
&P2&   \cellcolor{white!10}{0.00 (0.02)} & \cellcolor{white!10}{N$^\dagger$}
    &  \textbf{\cellcolor{blue!10}{0.04 (0.02)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \cellcolor{red!10}label timeout&\cellcolor{red!10}
    &  \cellcolor{white!10}{0.00 (0.04)} & \cellcolor{white!10}{N}
    &  \cellcolor{blue!10}{0.01 (0.04)} & \cellcolor{blue!10}{N}
    &  \textbf{\cellcolor{red!10}{$-$1.42 (0.27)}} & \textbf{\cellcolor{red!10}{L$^\dagger$}}\\



    
     
   \bottomrule
   
   %\quart{of 0}{16}{10}{20}
    %\rowcolor{blue!10}\textbf{5} & \textbf{D1} & \textbf{0.80} & \textbf{0.14} & \quart{71}{14}{80}{100}\\
\end{tabular}
%\end{adjustbox}
\end{table*}


==> Tables/chap-encoding/rq2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[!t]
\caption{The Scott-Knott test scores of the RMSE of the five subject systems; Each line represents the relative scoreings of the RMSE over 50 runs of each performance model with each encoding method. A higher scire means a lower RMSE, which means the results are better. If two results are of the same score, they have insignificant difference.}
\label{tb:rq2-acc}
\centering
\setlength{\tabcolsep}{0.9mm}
\begin{tabular}{@{}l|ccc|ccc|ccc|ccc|ccc|ccc|ccc@{}}
\toprule
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}DT} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}KNN} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}KRR} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}LR} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}NN} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}RF} &
  \multicolumn{3}{c}{\cellcolor[HTML]{FFFFFF}SVR} \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}} & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA \\
\rowcolor[HTML]{EFEFEF} 
MongoDB &
  6 &
  6 &
  6 &
  4 &
  3 &
  5 &
  9 &
  8 &
  8 &
  8 &
  8 &
  8 &
  10 &
  10 &
  10 &
  7 &
  8 &
  8 &
  2 &
  1 &
  1 \\
\rowcolor[HTML]{C0C0C0} 
Irzip &
  7 &
  9 &
  9 &
  4 &
  6 &
  5 &
  3 &
  2 &
  2 &
  2 &
  2 &
  2 &
  12 &
  10 &
  11 &
  7 &
  8 &
  8 &
  1 &
  1 &
  1 \\
\rowcolor[HTML]{EFEFEF} 
Trimesh &
  8 &
  7 &
  7 &
  6 &
  2 &
  5 &
  4 &
  3 &
  3 &
  3 &
  3 &
  3 &
  11 &
  12 &
  12 &
  9 &
  10 &
  10 &
  1 &
  1 &
  1 \\
\rowcolor[HTML]{C0C0C0} 
ExaStencils &
  11 &
  11 &
  11 &
  9 &
  8 &
  10 &
  10 &
  7 &
  5 &
  1 &
  2 &
  2 &
  14 &
  13 &
  13 &
  12 &
  12 &
  12 &
  6 &
  4 &
  3 \\
\rowcolor[HTML]{EFEFEF} 
X264-DB &
  14 &
  15 &
  11 &
  10 &
  5 &
  12 &
  13 &
  7 &
  6 &
  1 &
  9 &
  8 &
  19 &
  19 &
  17 &
  17 &
  18 &
  16 &
  3 &
  4 &
  2 \\ \bottomrule
\end{tabular}
\end{table*}

==> Tables/chap-encoding/rq3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[!t]
\caption{The Scott-Knott rank test results of the training time of the five subject systems; Each line represents the relative rankings of the training time over 50 runs of each performance model with each encoding method. A higher ranking means less training time, which means the results are better. If two results are of the same rank, they have insignificant difference.}
\label{tb:rq3-time}
\centering
\setlength{\tabcolsep}{0.9mm}
\begin{tabular}{@{}l|ccc|ccc|ccc|ccc|ccc|ccc|ccc@{}}
\toprule
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}DT} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}KNN} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}KRR} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}LR} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}NN} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}RF} &
  \multicolumn{3}{c}{\cellcolor[HTML]{FFFFFF}SVR} \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}} & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA \\
\rowcolor[HTML]{EFEFEF} 
MongoDB                                      & 13 & 17  & 16  & 14 & 15  & 12  & 6  & 2   & 8   & 18 & 19  & 19  & 10 & 7   & 11  & 1  & 9   & 4   & 3  & 5   & 1   \\
\rowcolor[HTML]{C0C0C0} 
Irzip                                        & 12 & 14  & 15  & 13 & 17  & 16  & 5  & 11  & 10  & 18 & 19  & 20  & 1  & 2   & 3   & 1  & 8   & 9   & 4  & 7   & 6   \\
\rowcolor[HTML]{EFEFEF} 
Trimesh                                      & 13 & 15  & 16  & 14 & 18  & 17  & 10 & 12  & 11  & 19 & 20  & 20  & 2  & 4   & 3   & 1  & 8   & 9   & 5  & 6   & 7   \\
\rowcolor[HTML]{C0C0C0} 
ExaStencils                                  & 12 & 14  & 15  & 13 & 17  & 16  & 10 & 4   & 11  & 18 & 19  & 20  & 5  & 2   & 3   & 1  & 9   & 8   & 5  & 6   & 7   \\
\rowcolor[HTML]{EFEFEF} 
X264-DB                                      & 11 & 17  & 15  & 12 & 16  & 14  & 7  & 10  & 6   & 13 & 19  & 18  & 3  & 5   & 8   & 2  & 4   & 3   & 1  & 5   & 9   \\ \bottomrule

\end{tabular}
\end{table*}

==> Tables/chap-meta/RQ1.tex <==
\begin{tabular}
{clp{0.3cm}c|p{0.2cm}c|p{0.2cm}c|p{0.2cm}c|p{0.2cm}c}
\toprule
                           &         & \multicolumn{2}{c}{\MetaModel}                                                    & \multicolumn{2}{c}{DeepPerf}               & \multicolumn{2}{c}{DECART}         & \multicolumn{2}{c}{RF}     & \multicolumn{2}{c}{SQLConqueror}             \\ \cline{3-12}
System &     & $r$                                & \multicolumn{1}{c}{Med (IQR)}                & $r$         & \multicolumn{1}{c}{Med (IQR)} & $r$         & Med (IQR)             & $r$      & Med (IQR)        & $r$         & Med (IQR)             \\ \hline
                           & Task 1  & {\cellcolor{green!20}\textbf{1}} & {\cellcolor{green!20}\textbf{17.56(1.75)}}  & 2          & 21.56(3.94)                   & 2          & 23.68(5.58)           & 2       & 24.95(6.27)      & 3          & 104.02(20.21)         \\
                           & Task 2  & {\cellcolor{green!20}\textbf{1}} & {\cellcolor{green!20}\textbf{11.26(1.01)}}  & 2          & 18.48(4.38)                   & 3          & 22.53(10.55)          & 3       & 22.09(8.20)      & 4          & 93.98(12.20)          \\
                           & Task 3  & {\cellcolor{green!20}\textbf{1}} & {\cellcolor{green!20}\textbf{17.61(3.57)}}  & 2          & 19.81(5.79)                   & 3          & 21.31(4.82)           & 3       & 21.94(7.30)      & 4          & 92.07(12.92)          \\
                           & Task 4  & {\cellcolor{green!20}\textbf{1}} & {\cellcolor{green!20}\textbf{14.48(2.44)}}  & 2          & 20.04(8.17)                   & 2          & 20.06(5.37)           & 3       & 21.30(5.93)      & 4          & 98.68(15.21)          \\
                           & Task 5  & {\cellcolor{green!20}\textbf{1}} & {\cellcolor{green!20}\textbf{9.98(1.50)}}   & 2          & 17.75(3.23)                   & 2          & 17.45(7.24)           & 3       & 22.82(7.60)      & 4          & 70.20(12.18)          \\
                           & Task 6  & {\cellcolor{green!20}\textbf{1}} & {\cellcolor{green!20}\textbf{9.99(1.21)}}   & 2          & 15.29(4.31)                   & 3          & 19.06(8.06)           & 3       & 18.87(7.42)      & 4          & 67.38(7.30)           \\
                           & Task 7  & {\cellcolor{green!20}\textbf{1}} & {\cellcolor{green!20}\textbf{11.07(1.94)}}  & 2          & 14.69(3.52)                   & 3          & 17.64(4.75)           & 2       & 15.88(5.81)      & 4          & 59.07(7.44)           \\
                           & Task 8  & {\cellcolor{green!20}\textbf{1}} & {\cellcolor{green!20}\textbf{6.78(0.84)}}   & 2          & 7.81(1.46)                    & 3          & 9.05(2.34)            & 2       & 7.45(2.11)       & 4          & 20.01(1.72)           \\
                           & Task 9  & {\cellcolor{green!20}\textbf{1}} & {\cellcolor{green!20}\textbf{10.47(1.36)}}  & 2          & 18.5(6.36)                    & 3          & 21.02(7.48)           & 3       & 21.08(10.03)     & 4          & 86.10(12.26)          \\
\multirow{-10}{*}{{x264}}    & Task 10 & {\cellcolor{green!20}\textbf{1}} & {\cellcolor{green!20}\textbf{12.08(2.22)}}  & 2          & 18.76(4.72)                   & 3          & 20.44(10.45)          & 3       & 21.18(7.58)      & 4          & 78.90(10.87)          \\ \hline
                           & Task 1  & 2                                 & 37.15(23.08)                                 & 3          & 45.7(24.91)                   & \textbf{1} & \textbf{30.57(19.40)} & 2       & 37.52(14.75)     & 4          & 84.69(8.98)           \\
                           & Task 2  & 3                                 & 77.87(16.57)                                 & 2          & 72.71(22.23)                  & \textbf{1} & \textbf{62.36(25.83)} & 3       & 74.90(16.70)     & 4          & 165.39(26.99)         \\
\multirow{-3}{*}{\textsc{DeepArch}} & Task 3  & {\cellcolor{green!20}\textbf{1}} & {\cellcolor{green!20}\textbf{36.52(10.60)}} & 2          & 40.76(7.65)                   & \textbf{1} & \textbf{34.53(12.09)} & 2       & 41.63(9.01)      & 3          & 109.68(21.53)         \\ \hline
                           & Task 1  & {\cellcolor{green!20}\textbf{1}} & {\cellcolor{green!20}\textbf{1.11(0.06)}}   & 2          & 1.14(0.12)                    & 4          & 1.58(0.12)            & 3       & 1.16(0.05)       & \textbf{1} & \textbf{1.11(0.05)}   \\
                           & Task 2  & {\cellcolor{green!20}\textbf{1}} & {\cellcolor{green!20}\textbf{1.05(0.06)}}   & 2          & 1.09(0.13)                    & 4          & 1.50(0.11)            & 3       & 1.11(0.04)       & 2          & 1.07(0.04)            \\
\multirow{-3}{*}{\textsc{SQLite}}   & Task 3  & 2                                 & 1.06(0.11)                                   & 2          & 1.04(0.08)                    & 4          & 1.49(0.10)            & 3       & 1.12(0.06)       & \textbf{1} & \textbf{1.03(0.05)}   \\ \hline
                           & Task 1  & {\cellcolor{green!20}\textbf{1}} & {\cellcolor{green!20}\textbf{804.37(901)}}  & \textbf{1} & \textbf{810.48(692)}          & 2          & 1506.57(923.87)       & 3       & 1670.97(766.66)  & 2          & 1554.03(366.39)       \\
                           & Task 2  & 2                                 & 41.62(28.78)                                 & 3          & 54.82(34.52)                  & \textbf{1} & \textbf{30.42(40.72)} & 4       & 56.70(30.24)     & 5          & 254.46(50.62)         \\
                           & Task 3  & 4                                 & 36.3(20.07)                                  & 3          & 32.55(15.49)                  & \textbf{1} & \textbf{18.44(13.38)} & 2       & 31.17(17.37)     & 5          & 116.05(44.06)         \\
                           & Task 4  & 2                                 & 34.56(23.69)                                 & 3          & 39.2(19.17)                   & \textbf{1} & \textbf{20.16(19.21)} & 3       & 39.23(13.54)     & 4          & 196.19(73.04)         \\
\multirow{-5}{*}{\textsc{SaC}}      & Task 5  & {\cellcolor{green!20}\textbf{1}} & {\cellcolor{green!20}\textbf{285.35(522)}}  & \textbf{1} & \textbf{256.81(250)}          & 2          & 737.16(1017.00)       & 3       & 2312.96(2921.64) & 4          & 10333.71(5601.18)     \\ \hline
                           & Task 1  & {\cellcolor{green!20}\textbf{1}} & {\cellcolor{green!20}\textbf{32.34(18.42)}} & 2          & 36.31(18.07)                  & 3          & 41.63(16.97)          & 3       & 41.06(12.17)     & \textbf{1} & \textbf{33.92(9.45)}  \\
                           & Task 2  & 2                                 & 58.09(10.63)                                 & 3          & 67.17(16.66)                  & 4          & 77.01(24.68)          & 4       & 74.90(16.70)     & \textbf{1} & \textbf{51.36(17.17)} \\
                           & Task 3  & {\cellcolor{green!20}\textbf{1}} & {\cellcolor{green!20}\textbf{25.59(11.58)}} & 3          & 36.2(16.63)                   & 3          & 37.99(9.65)           & 4       & 41.63(9.01)      & 2          & 28.88(5.48)           \\
                           & Task 4  & {\cellcolor{green!20}\textbf{1}} & {\cellcolor{green!20}\textbf{35.93(19.33)}} & 3          & 45.29(17.48)                  & 5          & 51.60(17.05)          & 4       & 48.07(12.37)     & 2          & 37.86(7.62)           \\
\multirow{-5}{*}{{gcc}}      & Task 5  & 3                                 & 45.0(21.09)                                  & 2          & 38.86(7.09)                   & 4          & 48.02(15.83)          & 3       & 43.97(10.13)     & \textbf{1} & \textbf{36.11(8.34)}  \\ \hline
                           & Task 1  & {\cellcolor{green!20}\textbf{1}} & {\cellcolor{green!20}\textbf{33.17(13.67)}} & 2          & 71.76(43.59)                  & 3          & 182.78(88.30)         & 4       & 237.25(41.13)    & 5          & 939.73(248.93)        \\
                           & Task 2  & {\cellcolor{green!20}\textbf{1}} & {\cellcolor{green!20}\textbf{27.15(7.83)}}  & \textbf{1} & \textbf{25.74(9.53)}          & 2          & 45.94(10.87)          & 2       & 47.58(6.35)      & 2          & 46.72(7.90)           \\
                           & Task 3  & 2                                 & 43.44(6.26)                                  & \textbf{1} & \textbf{36.89(3.17)}          & 3          & 57.60(10.08)          & 3       & 58.99(4.26)      & 4          & 645.18(258.51)        \\
                           & Task 4  & {\cellcolor{green!20}\textbf{1}} & {\cellcolor{green!20}\textbf{15.26(1.42)}}  & \textbf{1} & \textbf{16.84(2.07)}          & 2          & 31.19(7.19)           & 2       & 31.84(4.55)      & 2          & 37.29(7.59)           \\
                           & Task 5  & {\cellcolor{green!20}\textbf{1}} & {\cellcolor{green!20}\textbf{14.59(7.60)}}  & 2          & 31.65(5.07)                   & 3          & 51.90(10.52)          & 3       & 53.47(3.66)      & 4          & 556.09(230.75)        \\
\multirow{-6}{*}{\textsc{SPEAR}}    & Task 6  & {\cellcolor{green!20}\textbf{1}} & {\cellcolor{green!20}\textbf{4.65(2.01)}}   & 2          & 18.1(7.82)                    & 3          & 30.06(6.79)           & 3       & 31.14(2.71)      & 4          & 173.86(115.01)        \\ \hline
\multicolumn{2}{c}{Average $r$}        & 1.41                           & \multicolumn{1}{c}{}                         & 2.06     & \multicolumn{1}{c}{}          & 2.62      &                       & 2.91 &                  & 3.19     &                      \\
\bottomrule
\end{tabular}

==> Tables/chap-meta/RQ2.tex <==
\begin{tabular}{cccc|p{0.2cm}c|p{0.2cm}c|p{0.2cm}c|p{0.2cm}c|p{0.2cm}c}

\toprule
\multicolumn{1}{l}{}       &         & \multicolumn{2}{c}{\MetaModel}                                                    & \multicolumn{2}{c}{RF$_{SE}$}        & \multicolumn{2}{c}{LR$_{SE}$}       & \multicolumn{2}{c}{DeepPerf$_{PLUS}$}         & \multicolumn{2}{c}{RF$_{PLUS}$}      & \multicolumn{2}{c}{LR$_{PLUS}$} \\ \cline{3-14}
System                     &         & $r$                                & \multicolumn{1}{c}{Med (IQR)}                & $r$         & Med (IQR)             & $r$         & Med (IQR)             & $r$         & \multicolumn{1}{c}{Med (IQR)} & $r$         & Med (IQR)            & $r$      & Med (IQR)          \\

\hline
                           & Task 1  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{17.56(1.75)}}  & 3          & 47.15(27.98)          & 4          & 103.57(13.14)         & 2          & 21.56(3.94)                   & 5          & 203.05(8.51)         & 6       & 241.08(20.37)      \\
                           & Task 2  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{11.26(1.01)}}  & 3          & 24.80(12.23)          & 5          & 86.35(9.18)           & 2          & 18.48(4.38)                   & 3          & 24.07(1.24)          & 4       & 57.79(5.21)        \\
                           & Task 3  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{17.61(3.57)}}  & 3          & 21.02(9.30)           & 6          & 85.63(9.23)           & 2          & 19.81(5.79)                   & 4          & 24.14(1.04)          & 5       & 59.32(5.76)        \\
                           & Task 4  & 2                                 & 14.48(2.44)                                  & 4          & 23.18(3.28)           & 6          & 90.32(9.71)           & 3          & 20.04(8.17)                   & \textbf{1} & \textbf{12.23(1.00)} & 5       & 61.28(4.26)        \\
                           & Task 5  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{9.98(1.50)}}   & 3          & 24.96(6.10)           & 5          & 69.05(13.96)          & 2          & 17.75(3.23)                   & 4          & 30.57(2.23)          & 6       & 92.16(5.25)        \\
                           & Task 6  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{9.99(1.21)}}   & 2          & 11.58(2.40)           & 4          & 60.79(4.49)           & 3          & 15.29(4.31)                   & 2          & 11.82(0.50)          & 4       & 59.77(4.27)        \\
                           & Task 7  & 2                                 & 11.07(1.94)                                  & \textbf{1} & \textbf{9.14(1.20)}   & 4          & 54.14(5.02)           & 3          & 14.69(3.52)                   & 2          & 10.15(1.68)          & 5       & 65.70(3.93)        \\
                           & Task 8  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{6.78(0.84)}}   & 4          & 59.45(2.35)           & 3          & 19.62(1.55)           & 2          & 7.81(1.46)                    & 5          & 82.93(11.16)         & 6       & 139.97(13.54)      \\
                           & Task 9  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{10.47(1.36)}}  & 2          & 12.64(1.79)           & 6          & 78.81(7.99)           & 3          & 18.5(6.36)                    & 4          & 27.67(0.54)          & 5       & 56.99(3.32)        \\
\multirow{-10}{*}{\textsc{x264}}    & Task 10 & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{12.08(2.22)}}  & 2          & 14.50(3.02)           & 4          & 73.62(7.60)           & 3          & 18.76(4.72)                   & 2          & 14.70(0.88)          & 4       & 79.63(5.65)        \\ \hline
                           & Task 1  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{37.15(23.08)}} & 2          & 42.23(1.47)           & 4          & 178.18(1.20)          & 2          & 45.7(24.91)                   & 3          & 85.26(0.56)          & 3       & 85.10(9.94)        \\
                           & Task 2  & 3                                 & 77.87(16.57)                                 & \textbf{1} & \textbf{33.29(2.18)}  & 4          & 102.24(2.32)          & 3          & 72.71(22.23)                  & 2          & 56.71(0.32)          & 5       & 160.27(35.62)      \\
\multirow{-3}{*}{\textsc{DeepArch}} & Task 3  & 2                                 & 36.52(10.60)                                 & \textbf{1} & \textbf{29.71(0.56)}  & 5          & 156.31(1.78)          & 2          & 40.76(7.65)                   & 3          & 66.88(0.44)          & 4       & 105.89(26.38)      \\ \hline
                           & Task 1  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{1.11(0.06)}}   & 5          & 1.92(0.74)            & \textbf{1} & \textbf{1.12(0.02)}   & 2          & 1.14(0.12)                    & 3          & 1.25(0.02)           & 4       & 1.31(0.17)         \\
                           & Task 2  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{1.05(0.06)}}   & 5          & 1.42(1.02)            & \textbf{1} & \textbf{1.05(0.02)}   & 2          & 1.09(0.13)                    & 3          & 1.16(0.02)           & 4       & 1.26(0.18)         \\
\multirow{-3}{*}{\textsc{SQLite}}   & Task 3  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{1.06(0.11)}}   & 3          & 2.10(1.40)            & \textbf{1} & \textbf{1.05(0.01)}   & \textbf{1} & \textbf{1.04(0.08)}           & 2          & 1.20(0.02)           & 2       & 1.26(0.19)         \\ \hline
                           & Task 1  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{804.37(901)}}  & 5          & 3608.43(855.82)       & 3          & 2985.80(492.52)       & \textbf{1} & \textbf{810.48(692)}          & 4          & 3141.48(666.24)      & 2       & 1328.54(401.31)    \\
                           & Task 2  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{41.62(28.78)}} & 3          & 175.05(4.73)          & 5          & 272.15(19.89)         & 2          & 54.82(34.52)                  & 4          & 248.43(12.69)        & 6       & 300.84(73.80)      \\
                           & Task 3  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{36.3(20.07)}}  & 2          & 177.48(5.41)          & 3          & 188.42(5.57)          & \textbf{1} & \textbf{32.55(15.49)}         & 2          & 178.33(1.80)         & 3       & 183.86(47.09)      \\
                           & Task 4  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{34.56(23.69)}} & 6          & 367.55(4.00)          & 3          & 229.08(4.88)          & 2          & 39.2(19.17)                   & 4          & 240.60(4.28)         & 5       & 297.67(74.96)      \\
\multirow{-5}{*}{\textsc{SaC}}      & Task 5  & { \textbf{2}} & 485.35(522)                                  & 6          & 32941.14(2481.96)     & 4          & 22544.21(2302.91)     & \textbf{1} & \textbf{256.81(250)}          & 5          & 25114.39(1909.88)    & 3       & 6759.09(3883.93)   \\ \hline
                           & Task 1  & 2                                 & 32.34(18.42)                                 & 2          & 33.42(4.93)           & \textbf{1} & \textbf{30.55(7.77)}  & 3          & 36.31(18.07)                  & 4          & 12473.23(1112.81)    & 4       & 11823.40(1037.05)  \\
                           & Task 2  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{58.09(10.63)}} & \textbf{1} & \textbf{56.22(13.88)} & \textbf{1} & \textbf{59.15(18.98)} & 2          & 67.17(16.66)                  & 3          & 14174.05(2119.32)    & 3       & 13472.99(1935.50)  \\
                           & Task 3  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{25.59(11.58)}} & 2          & 29.91(5.10)           & 3          & 31.00(7.82)           & 4          & 36.2(16.63)                   & 5          & 681.30(58.27)        & 5       & 641.02(49.80)      \\
                           & Task 4  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{35.93(19.33)}} & 2          & 42.66(6.78)           & 2          & 41.07(13.11)          & 3          & 45.29(17.48)                  & 4          & 69.28(3.41)          & 4       & 64.82(3.60)        \\
\multirow{-5}{*}{\textsc{gcc}}      & Task 5  & 3                                 & 45.0(21.09)                                  & 3          & 44.26(10.55)          & 2          & 41.61(14.87)          & \textbf{1} & \textbf{38.86(7.09)}          & 5          & 50.34(5.39)          & 4       & 46.69(5.76)        \\ \hline
                           & Task 1  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{33.17(13.67)}} & 4          & 1078.39(4.53)         & 3          & 633.85(1.78)          & 2          & 71.76(43.59)                  & 3          & 672.80(1.41)         & 4       & 1019.54(335.29)    \\
                           & Task 2  & 2                                 & 27.15(7.83)                                  & 4          & 40.92(0.42)           & 5          & 43.21(0.09)           & \textbf{1} & \textbf{25.74(9.53)}          & 3          & 38.42(0.06)          & 6       & 53.04(8.61)        \\
                           & Task 3  & 2                                 & 43.44(6.26)                                  & 6          & 826.89(2.86)          & 4          & 528.18(1.16)          & \textbf{1} & \textbf{36.89(3.17)}          & 3          & 397.27(0.49)         & 5       & 742.93(259.66)     \\
                           & Task 4  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{15.26(1.42)}}  & 4          & 24.53(0.32)           & 5          & 34.83(0.09)           & 2          & 16.84(2.07)                   & 3          & 21.64(0.03)          & 6       & 43.20(11.18)       \\
                           & Task 5  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{14.59(7.60)}}  & 6          & 706.01(2.25)          & 4          & 425.18(1.18)          & 2          & 31.65(5.07)                   & 3          & 335.31(0.49)         & 5       & 615.38(224.06)     \\
\multirow{-6}{*}{{SPEAR}}    & Task 6  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{4.65(2.01)}}   & 6          & 266.18(0.44)          & 4          & 149.45(0.48)          & 2          & 18.1(7.82)                    & 3          & 108.49(0.17)         & 5       & 194.86(138.94)     \\
\hline
\multicolumn{2}{c}{Average $r$}        & 1.34                           & \multicolumn{1}{c}{}                         & 3.31     &                       & 3.59    &                       & 2.09    & \multicolumn{1}{c}{}          & 3.31     &                      & 4.43  &                   \\
\bottomrule
\end{tabular}

==> Tables/chap-meta/RQ3.tex <==
\begin{tabular}{clcc|p{0.2cm}c|p{0.2cm}c|p{0.2cm}c|p{0.2cm}c}
\toprule
\multicolumn{1}{l}{}       &         & \multicolumn{2}{c}{\MetaModel}                                                   & \multicolumn{2}{c}{MAML}          & \multicolumn{2}{c}{MetaSGD}     & \multicolumn{2}{c}{RF$_{MTL}$}      & \multicolumn{2}{c}{BEETLE}       \\ \cline{3-12}
System                     &         & $r$                                & Med (IQR)                                   & $r$         & Med (IQR)            & $r$         & Med (IQR)          & $r$         & Med (IQR)           & $r$         & Med (IQR)           \\ \hline
                           & Task 1  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{17.56(1.75}}  & \textbf{1} & \textbf{17.34(1.62}  & 3          & 18.72(2.64         & 4          & 22.11(5.94          & 2          & 17.72(6.81          \\
                           & Task 2  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{11.26(1.01}}  & 2          & 11.57(1.23           & 2          & 11.53(1.81         & 4          & 18.44(3.24          & 3          & 12.62(1.27          \\
                           & Task 3  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{17.61(3.57}}  & 4          & 20.65(3.38           & 3          & 19.77(5.11         & 5          & 23.43(8.12          & 2          & 18.14(3.87          \\
                           & Task 4  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{14.48(2.44}}  & 3          & 16.11(2.87           & 3          & 16.73(1.87         & 4          & 22.39(2.98          & 2          & 15.01(4.77          \\
                           & Task 5  & 2                                 & 9.98(1.50                                   & 4          & 14.15(5.76           & 3          & 10.98(5.58         & \textbf{1} & \textbf{9.76(1.75}  & 2          & 10.09(1.69          \\
                           & Task 6  & 2                                 & 9.99(1.21                                   & 4          & 14.81(2.91           & 4          & 14.59(2.69         & 3          & 10.50(1.37          & \textbf{1} & \textbf{9.79(1.16}  \\
                           & Task 7  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{11.07(1.94}}  & 2          & 11.14(1.48           & 3          & 12.15(2.99         & 2          & 11.30(1.91          & 3          & 12.15(1.04          \\
                           & Task 8  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{6.78(0.84}}   & 2          & 7.39(1.77            & \textbf{1} & \textbf{6.81(0.98} & 3          & 8.19(1.67           & 2          & 7.09(4.34           \\
                           & Task 9  & 2                                 & 10.47(1.36                                  & 3          & 12.18(1.46           & 4          & 13.21(1.16         & 5          & 16.42(2.16          & \textbf{1} & \textbf{9.95(2.68}  \\
\multirow{-10}{*}{\textsc{x264}}    & Task 10 & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{12.08(2.22}}  & 5          & 20.06(3.64           & 3          & 13.69(2.96         & 4          & 15.34(8.13          & 2          & 12.48(2.02          \\ \hline
                           & Task 1  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{37.15(23.08}} & 2          & 44.15(25.21          & 2          & 45.49(7.87         & 3          & 66.6(7.92           & \textbf{1} & \textbf{36.96(9.67} \\
                           & Task 2  & 4                                 & 77.87(16.57                                 & \textbf{1} & \textbf{45.76(13.57} & 2          & 49.39(7.72         & 5          & 84.41(6.5           & 3          & 67.78(15.32         \\
\multirow{-3}{*}{\textsc{DeepArch}} & Task 3  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{36.52(10.60}} & 2          & 38.62(5.91           & 2          & 37.58(2.98         & \textbf{1} & \textbf{35.43(6.71} & 3          & 41.07(8.71          \\ \hline
                           & Task 1  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{1.11(0.06}}   & \textbf{1} & \textbf{1.11(0.13}   & 2          & 1.18(0.15          & 3          & 7.11(0.77           & 2          & 1.14(0.66           \\
                           & Task 2  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{1.05(0.06}}   & 2          & 1.09(0.12            & 3          & 1.13(0.25          & 4          & 1.72(0.06           & 2          & 1.07(0.12           \\
\multirow{-3}{*}{\textsc{SQLite}}   & Task 3  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{1.06(0.11}}   & 3          & 1.15(0.07            & 5          & 1.31(0.16          & 4          & 1.20(0.05           & 2          & 1.08(0.33           \\ \hline
                           & Task 1  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{804.37(901}}  & 5          & 1819(891             & 3          & 1135(974           & 4          & 1331(748            & 2          & 945(491             \\
                           & Task 2  & 2                                 & 41.62(28.78                                 & 4          & 62.91(26.89          & 3          & 52.30(36.8         & 5          & 90.68(26.5          & \textbf{1} & \textbf{40.97(9.95} \\
                           & Task 3  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{36.3(20.07}}  & 4          & 120.66(50.97         & 3          & 83.89(35.01        & 5          & 279.80(84.55        & 2          & 72.0(15.87          \\
                           & Task 4  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{34.56(23.69}} & 3          & 98.10(34.11          & 2          & 64.81(20.62        & 4          & 162.15(82.15        & 5          & 208.71(55.46        \\
\multirow{-5}{*}{\textsc{SaC}}      & Task 5  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{485.35(522}}  & 2          & 839.1(529            & 5          & 4163(969           & 3          & 2022(343            & 4          & 3495(732            \\ \hline
                           & Task 1  & 2                                 & 32.34(18.42                                 & 2          & 36.68(20.39          & 3          & 42.33(29.7         & \textbf{1} & \textbf{28.29(18.8} & 4          & 57.43(15.74         \\
                           & Task 2  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{58.09(10.63}} & 4          & 95.76(20.3           & 2          & 66.03(22.8         & 3          & 88.67(32.9          & \textbf{1} & \textbf{57.27(9.33} \\
                           & Task 3  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{25.59(11.58}} & 3          & 49.07(26.12          & 4          & 55.00(28.64        & 3          & 46.02(19.58         & 2          & 33.70(8.33          \\
                           & Task 4  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{35.93(19.33}} & 3          & 57.14(27.18          & 3          & 60.38(18.13        & 4          & 71.75(18.88         & 2          & 43.52(10.6          \\
\multirow{-5}{*}{\textsc{gcc}}      & Task 5  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{45.0(21.09}}  & 3          & 60.95(20.61          & 3          & 57.46(13.67        & 4          & 73.09(28.37         & 2          & 46.47(16.39         \\ \hline
                           & Task 1  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{33.17(13.67}} & 3          & 44.20(16.28          & 4          & 57.15(15.38        & 5          & 78.10(10.55         & 2          & 37.65(8.01          \\
                           & Task 2  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{27.15(7.83}}  & 3          & 31.92(12.2           & 3          & 31.97(14.15        & 2          & 29.18(17.68         & 3          & 30.96(19.43         \\
                           & Task 3  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{43.44(6.26}}  & 2          & 44.52(5.25           & 2          & 45.64(5.7          & 2          & 48.23(13.64         & 3          & 61.89(20.3          \\
                           & Task 4  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{15.26(1.42}}  & 4          & 17.46(4.53           & 3          & 16.66(6.36         & 4          & 19.41(4.07          & 2          & 15.56(3.14          \\
                           & Task 5  & 2                                 & 14.59(7.60                                  & 3          & 24.19(14.65          & 4          & 29.14(15.53        & 4          & 28.13(9.43          & \textbf{1} & \textbf{13.55(2.9}  \\
\multirow{-6}{*}{\textsc{SPEAR}}    & Task 6  & {\cellcolor{green!20} \textbf{1}} & {\cellcolor{green!20} \textbf{4.65(2.01}}   & 5          & 7.69(1.84            & 4          & 6.028(1.86         & 3          & 5.85(1.61           & 2          & 4.72(1.22           \\ \hline
\multicolumn{2}{c}{Average $r$}        & 1.28                           &                                             & 2.94     &                      & 3          &                    & 3.47    &                     & 2.219    &                    \\ 
\bottomrule
\end{tabular}

==> Tables/chap-meta/algorithm.tex <==
\begin{algorithm}[t!]
	\DontPrintSemicolon
	\footnotesize
	
	\caption{Pseudo code of \MetaModel}
	\label{chap-meta-alg:code}
	\KwIn{A group of related tasks $\mathbfcal{\overline{T}}=\mathbf{(\overline{x}, \overline{y})}$; a set of training samples $\mathbfcal{S}=\mathbf{\overline{x}}$; a new set of configurations $\mathbf{\overline{x}}$ to be predicted}
     \KwOut{The predicted performance of $\mathbf{\overline{x}}$}
    %\KwOut{A set of division-dedicated models $\mathbfcal{M}$}
	%\kwDeclare{$\Delta=0.1$; bounds of weight: $w_{max}=10^3$; $w_{min}=0$}
	
\If{$\mathbfcal{M} = \emptyset$}
	{
	  \tcc{\textcolor{blue}{dividing phase.}}
      $\mathbfcal{S}\leftarrow$ randomly sample a set of configurations and their performance\\
      $\mathcal{T}\leftarrow$ \textsc{trainCART($\mathbfcal{S}$)}\\
      $d'=1$\\
      \While{$d'\leq d$}{
           \If{$d'<d$}
           {
             $\mathbfcal{D}\leftarrow$ extract all the leaf divisions of samples from $\mathcal{T}$ at the $d'$th depth\\
           }
           \Else{
              $\mathbfcal{D}\leftarrow$ extract all divisions of samples from $\mathcal{T}$ at the $d'$th depth\\
           }
           $d'=d'+1$\\
      }
      
      %$\mathbfcal{D}\leftarrow$ extract the divisions of data samples from $\mathcal{T}$ at the $d$th depth\\
      \tcc{\textcolor{blue}{training phase.}}
      \For{$D_i \in \mathbfcal{D}$}  
      {
       $\mathbfcal{M}\leftarrow$ \textsc{trainDNN($D_i$)}\\
    
      }
    
    }
       
    \tcc{\textcolor{blue}{predicting phase.}}
    \If{$\mathcal{F}$ has not been trained}
	{
	$\mathbfcal{U}\leftarrow$ Removing performance data and labeling the configurations based on their divisions in $\mathbfcal{D}$\\
	$\mathbfcal{U'}\leftarrow$ \textsc{SMOTE($\mathbfcal{U}$)}\\
	$\mathcal{F}\leftarrow$ \textsc{trainRandomForest($\mathbfcal{U'}$)}
	}
	
    $D_i=$  \textsc{predict($\mathcal{F}$,$\mathbf{\overline{c}}$)}\\
    $\mathcal{M}=$ get the model from $\mathbfcal{M}$ that corresponds to the predicted division $D_i$\\ 
       
    

    \Return \textsc{predict($\mathcal{M}$,$\mathbf{\overline{c}}$)}\\
	
\end{algorithm}

==> Tables/chap-meta/data_example.tex <==
% \begin{table}[]
% \centering
% \small
% \caption{An example of performance dataset. $\overline{x}$ are the configurations and $\varmathbb{P}$ is the performance value.}
\begin{tabular}{lllllll||c||c}
\toprule
$x_{1}$ & $x_{2}$ & $x_{3}$ & $\cdots$ & $x_{n-2}$ & $x_{n-1}$ & $x_{n}$ & $\mathcal{P}_{1}$ & $\mathcal{P}_{2}$\\ \midrule
0 & 0 & 0 & $\cdots$ & 0 & 3 & 10 & 1200 seconds & 1400 seconds\\ 
0 & 1 & 0 & $\cdots$ & 0 & 2 & 11 & 2100 seconds & 3000 seconds\\ 
$\cdots$        & $\cdots$  & $\cdots$       & $\cdots$       & $\cdots$       & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$\\ 
0 & 0 & 1 & $\cdots$ & 0 & 9 & 23 & 1260 seconds & 1400 seconds\\ 
0 & 0 & 1 & $\cdots$ & 1 & 8 & 65 & 1140 seconds & 2200 seconds\\ \bottomrule
\end{tabular}
% \label{tb:data_example}
% \end{table}

==> Tables/chap-meta/subject_system.tex <==
\begin{table}[t!]
\caption{Details of the subject systems. $|\mathbfcal{T}|$ denotes the number of tasks in the dataset, ($|\mathbfcal{B}|$/$|\mathbfcal{N}|$) denotes the number of binary/numerical options, and $|\mathbfcal{C}|$ denotes the number of valid configurations (full sample size).}
\centering
\footnotesize
\begin{adjustbox}{width=\linewidth,center}
\begin{tabular}{cccccc}
\toprule

\textbf{Dataset} & \textbf{Description} & \textbf{$|\mathbfcal{T}|$} & \textbf{$|\mathbfcal{B}|$/$|\mathbfcal{N}|$} & \textbf{$|\mathbfcal{C}|$}  & \textbf{Used by}         \\
\midrule
\textsc{SaC}      & Cloud tool     & 3       & 58/0             & 4999  & \citet{DBLP:journals/corr/abs-1911-01817}          \\
\textsc{SQLite}   & DBMS           & 3       & 14/0             & 1000  & \citet{DBLP:journals/corr/abs-1911-01817}          \\
\textsc{SPEAR}    & Audio editing  & 6       & 14/0             & 16385 & \citet{DBLP:journals/corr/abs-1911-01817}          \\
\textsc{DeepArch} & DNN tool       & 3       & 12/0             & 4096  & \citet{DeepArch-Xplorer} \\
\textsc{x264}     & Vedio encoding & 10      & 11/13            & 201   & \citet{DBLP:journals/corr/abs-2112-07279}      \\
\textsc{GCC}      & Compilation    & 5       & 5/0              & 81    & \citet{DBLP:journals/corr/abs-2112-07279}     \\

\bottomrule
\end{tabular}
\end{adjustbox}
\label{chap-meta-table:subject systems}
\end{table}

==> cover_letter_revision.tex <==
% \section{Cover Letter}

% \begin{flushleft} 
% Dear Hui and Pooyan,
% \end{flushleft} 

% I hope you are all well. I am writing to formally submit the revised final version of my PhD thesis, titled ``Pushing the Boundary: Specialising Deep Configuration Performance Learning'', in accordance with the required corrections discussed during the viva examination conducted on 15th March 2024.

% I would like to express my sincere gratitude for your valuable feedback and constructive suggestions. I have diligently addressed each comment, suggestion, and correction in the relevant sections of the thesis. A detailed summary of the revisions made is as follows:


% \begin{enumerate}
% \item \textbf{Comment:} Rephrase the sentence in the first paragraph in the abstract.

% \begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt]{\textbf{Revision:}} Thank you for your valuable suggestion. I have revised the first paragraph of the abstract to address that deep learning models have been utilized due to their ability to learn meaningful representations from limited data, which is exactly one of the key challenges in configuration performance modeling.
% \end{tcolorbox}



% \item \textbf{Comment:} Shorten the chapter 2.

% \begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt]{\textbf{Revision:}} Thank you for your advice. I have shortened the methodology chapter (Chaper~\ref{chap:methodology}) by simplifying the backgrounds and introductions of the methodology. Particularly, the length of the chapter has been reduced from 10 pages to 7 pages.
% \end{tcolorbox}



% \item \textbf{Comment:} Remove a para on page 2.

% \begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt]{\textbf{Revision:}} Thank you for your feedback. I have removed the redundant paragraph accordingly in the introduction (Section~\ref{chap:introduction}).
% \end{tcolorbox}



% \item \textbf{Comment:} Replace the x bar on page 3.

% \begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt]{\textbf{Revision:}} Good suggestion! I have replaced the $\times$ mark with ``times'' in Section~\ref{chap:introduction}.
% \end{tcolorbox}



% \item \textbf{Comment:} change the subscript of Eq. 1.3.

% \begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt]{\textbf{Revision:}} Thank you for your helpful suggestion. To avoid confusion of $\overline{x}$ with $x$, I have changed the symbol of configuration to $\mathbf{c}$, where $\mathbf{c}=\{x_1,x_2,...,x_n\}$ as presented in Section~\ref{chap-intro:deep_learning}.
% \end{tcolorbox}



% \item \textbf{Comment:} Page 5. typo.

% \begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt]{\textbf{Revision:}} Thank you very much. I have revised the typo.
% \end{tcolorbox}



% \item \textbf{Comment:} Page 28. put real number there.

% \begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt]{\textbf{Revision:}} Thank you for your valuable comment. I have added the actual number of studies for each finding in the systematic literature review, as can be seen in Section~\ref{chap-survey:contributions}.
% \end{tcolorbox}



% \item \textbf{Comment:} Page 32. table 3.1. change the data item to something else to avoid confusion.

% \begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt]{\textbf{Revision:}} That is a very good point! Thank you. To avoid confusion, I have changed the term ``data item'' to ``review element'', and replaced the symbol ``$I_{x}$'' with ``$E_{x}$'' as shown in Table~\ref{tb:data_items}.
% \end{tcolorbox}



% \item \textbf{Comment:} Page 35 table 3.2. make the embedding, oversampling more specific.

% \begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt]{\textbf{Revision:}} Thank you for your careful review. I have reviewed the studies again and updated the preprocessing techniques, i.e., the general terms ``oversampling'' and ``embedding'' have been replaced with specific techniques like ``SMOTUNED'' and ``graph embedding'' in Table~\ref{tb:preprocessing}. Moreover, the corresponding introductions of the preprocessing methods have also been rephrased.
% \end{tcolorbox}



% \item \textbf{Comment:} Reprhase the featurization section.

% \begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt]{\textbf{Revision:}} Thank you, the original section for featurization is indeed confusing. I have changed the category name ``featurization'' to ``feature construction'', and rewritten the descriptions of these techniques accordingly, as can be found in Table~\ref{tb:preprocessing}.
% \end{tcolorbox}



% \item \textbf{Comment:} Justify why the encoding schemes are split from preprocessing stage.

% \begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt]{\textbf{Revision:}} Very good point, thank you for your insightful suggestion! I have justified this in Section~\ref{chap-survey:how-to-encode}. Specifically, after data preprocessing, the configuration data may still remains in the format of natural language, including binary options like ``yes/no'' or ``on/off'', as well as categorical options such as ``low/medium/high quality''. In such cases, it is often essential to apply suitable encoding schemes to further convert the configuration data into a more appropriate format for deep learning. Thereby, this process stands out as a fundamental step alongside other preprocessing methods. 
% \end{tcolorbox}



% \item \textbf{Comment:} 1. Table 3.4. put residual neural network under CNN.

% 2. Restructure some items in Tabl3.4

% \begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt]{\textbf{Revision:}} Thank you very much for the advice. I have re-grouped the deep learning models according to your comments during the viva and listed the number of studies for each specific model in Table~\ref{tb:learning}. Additionally, the entire Section~\ref{chap-survey:what-deep-learning} has been rephrased based on the new table.
% \end{tcolorbox}




% \item \textbf{Comment:} 1. On page 49, please check the omitted category.

% 2. On page 65, please double-check if the 46 studies used standard settings or just really forgot discussing the implementation details.

% \begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt]{\textbf{Revision:}} Thank you for your constructive comment. After careful double-checking, I am highly confident that these studies have not provided information about optimization methods and activation functions in any format. Therefore, it is reasonable to assume that the authors should have utilized the default settings from the implementation library. Nonetheless, I believe it is necessary to keep these studies as an individual category instead of grouping them according to a standard, because it is always a good behavior to provide the implementing details or source codes for better understanding and replication. 

% As such, I have changed the term ``omitted'' to ``default'' in Figure~\ref{subfig:optimization} and Figure~\ref{subfig:activation}, and have added justification on this in Section~\ref{chap-survey:optimization-and-activation}
% \end{tcolorbox}



% \item \textbf{Comment:} add some discussion on the hold-out experimental setting.

% \begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt]{\textbf{Revision:}} Thank you for the insightful suggestion. I have added more discussions in Section~\ref{chap-survey:evaluation-and-accuracy}. Specifically, hold-out evaluation involves splitting the dataset into training and testing sets based on a specific percentage. While hold-out is easy to implement and fast in evaluation overhead, it only evaluates the artifact once and is sensitive to the particular random split of the data, making the results bias and less reliable.

% On the other hand, cross-validation involves iteratively partitioning the dataset into multiple subsets for training and testing. To address the issues of hold-out, cross-validation makes multiple partitions similar to hold-out and computes the average performance, eventually utilizing the entire dataset for training and testing, which is efficient in the usage of data and offers better reliability.
% \end{tcolorbox}



% \item \textbf{Comment:} justify why the min-max scaling is used for the investigation of encoding schemes.

% \begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt]{\textbf{Revision:}} Good point! It is worth noting that min-max scaling is only applied for scaled label encoding, which normalizes the configuration options between 0 and 1. I have clarified the reasons for choosing min-max scaling in Section~\ref{chap-encoding:pipeline_setting}. In particular, min-max scaling is chosen because (1) it is computationally efficient, (2) it is easy to understand and implement, and (3) according to our systematic literature review in Section~\ref{subsec: preprocess}, max-min scaling is the most commonly-used normalization technique, used in 25 out of 32 studies.
% \end{tcolorbox}



% \item \textbf{Comment:} Page 86, rephrase the sentence to clarify that both machine learning and deep learning are used.

% \begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt]{\textbf{Revision:}} Thank you for your careful review. I have changed the confusing expressions in Section~\ref{chap-encoding:learning_models}. Particularly, the reasons for evaluating other machine learning models such as \texttt{RF} and \texttt{LR} in addition to deep neural networks in that chapter are two-fold: (1) they have been widely used in previous works for configuration performance learning, therefore ensure a better generalizability of the findings about encoding schemes, and (2) they exist in standard implementation under the same and widely-used machine learning library, i.e., \texttt{Sklearn} and \texttt{Tensorflow}, which reduces the possibility of bias.
% \end{tcolorbox}



% \item \textbf{Comment:} Make some discussion on how decision tree boundary will make impact on the samples located in some very sparse regions.

% \begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt]{\textbf{Revision:}} Very good advice! I have added further discussions on the influence of the decision boundaries for the sparse regions in Section~\ref{subsec:modeify-cart}.

% Specifically, the dividing process with \texttt{CART} are visualized in Figure~\ref{fig:3d-exp}, where the original dataset is divided into more focused divisions according to one or two most important configuration options based on the decision boundaries of \texttt{CART} and the parameter $d$. Nonetheless,  it is important to note that in some extremely sparse regions, an incorrect choice of $d$ may lead to samples with different characteristics and performance ranges being grouped together. For example, in Figure~\ref{fig:depth-nginx}, the division with \texttt{keepalive}=0 still exhibits sparse performance, indicating the need for further splitting using other decision boundaries provided by \texttt{CART}. As such, it is intuitive to understand that $d$ is such a critical parameter for \Model, and the necessity of an adaptive mechanism within \Model~that can enable dynamic adaptation of the $d$ value.

% Despite this, it is worth highlighting that even in such scenarios, the division where \texttt{keepalive}=1 displays a highly concentrated sample distribution, which can be effectively captured by the local model. 
% \end{tcolorbox}



% \item \textbf{Comment:} Update the text of DNN to a more generic term since they can be any base models.

% \begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt]{\textbf{Revision:}} Thank you for your valuable feedback! Indeed, the usage of \texttt{DNN} in Figure~\ref{fig:dal-structure} omits the advantage of \Model~that the base model can be any machine learning model. I have added extra explanation in the caption to clarify that the framework is model-agnostic.

% However, I would like to kindly note that since the default learner for \Model~is \texttt{DNN} (because it has the best performance in the experiments), I think it is reasonable to keep the figure that way to offer readers a more straightforward impression, and when they read to the RQ2 they will understand clearly why \Model~is flexible with base learner.
% \end{tcolorbox}



% \item \textbf{Comment:} For DaL\_Cart, what is the difference with CART model? Please clarify it.

% \begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt]{\textbf{Revision:}} That is a very interesting point! By using \texttt{CART} as the local model for \Model, the learning procedures would like very similar to the original \texttt{CART}. However, when looking at the results in Table~\ref{chap-dal-tb:compare_models}, we can see that \Model$_{CART}$ remains slightly better than using \texttt{CART} as the global model alone. This is possible due to two reasons: (1) \Model~adapts different techniques to assist the learning process, i.e., min-max scalling to normalize the configuration options, and SMOTE for over-sampling, which could affect the predictions, and (2) the actual result of the computed loss can be different in \texttt{CART} when it is presented with different proportions of the data samples. Yet, the resulting MREs do not differ much, as can be seen. The above clarifications have been added in Section~\ref{chap-meta-subsec:local}.
% \end{tcolorbox}



% \item \textbf{Comment:} use xgboost as a local model and see what the performance would be.

% \begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt]{\textbf{Revision:}} Thank you for your constructive comments. To address this problem, I have conducted further experiments on comparing \texttt{XGBoost} and \Model~with \texttt{XGBoost} as local learner (denoted as \Model$_{XGB}$), and the results have been added in Table~\ref{chap-dal-tb:compare_models}. 

% In particular, it can be seen that while \texttt{XGBoost} has better results for \textsc{SQLite}, \Model$_{XGB}$ performs significantly better or similar for most of the other software systems, especially for \textsc{Lrzip} and \textsc{nginx}. Furthermore, \Model$_{XGB}$ achieves an average rank of 3.63 over all systems and sample sizes, which is the 4th best rank among all the models in Table~\ref{chap-dal-tb:compare_models}, and 19.8\% better than the rank of 4.28 for \texttt{XGBoost}.
% \end{tcolorbox}



% \item \textbf{Comment:} Make Figure 6.7 clearer on annotation. Particularly, putting the explanation of figure details in annotations.

% \begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt]{\textbf{Revision:}} Thank you for your feedback. I have added detailed explanations in the captions of Figure~\ref{fig:rq1-mean}, Figure~\ref{fig:rq2-mean} and Figure~\ref{fig:rq3-mean}.
% \end{tcolorbox}



% \item \textbf{Comment:} add some discussions about the preservation of previous environment knowledge in sequential learning in
% future work.

% \begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt]{\textbf{Revision:}} Thank you for your insightful suggestion. I have added discussions on the utilization of incremental learning and lifelong learning techniques in Section~\ref{chap-meta:future_work}.
% \end{tcolorbox}



% \item \textbf{Comment:} discuss the impact of the fine-tuning stage after the meta-learning.

% \begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt]{\textbf{Revision:}} Thank you very much for the helpful comment. In Section~\ref{chap-meta:fine-tuning}, I have added further discussions on the impact of the fine-tuning stage.

% Notably, while the pre-trained meta-model demonstrates good generalizability and can be directly used for predicting configuration performance, the fine-tuning process is still necessary for the following reasons: (1) during fine-tuning, a critical step is to normalize the configuration options between 0 and 1, yet without fine-tuning, normalization would not be feasible, potentially leading to reduced prediction accuracy; (2) without fine-tuning, the meta-model can only use the default hyperparameters such as the learning rate and lambda for L1 regularization, which would also constraint its capabilities. In the subsequent experiment section, it will be further demonstrated that even with only a few fine-tuning samples, \MetaModel~is able to outperform the state-of-the-art configuration performance prediction models.
% \end{tcolorbox}

% \end{enumerate}

% Further to the comments, the additional updates made to the thesis can be summarized below:

% \begin{itemize}
%     \item I have comprehended the table captions and figure captions to make them readable on their own.

%     \item I have updated the status of the submitted papers, i.e., the new publication in FSE'24, and the re-submissions of the two journal papers in Table~\ref{chap1:publication} and Table~\ref{chap-conc-tb:summary}.

%     \item A new figure has been added to demonstrate the popularity of deep learning studies for software configuration performance learning (Figure~\ref{chap-review-fig:year_publications}).
% \end{itemize}


% These revisions have significantly strengthened the overall coherence and quality of this thesis. Thank you again for your professional review and guidance.

% I look forward to receiving any further instructions or feedback regarding the submission of the revised thesis.



% % \vspace{-1cm}
% \begin{flushleft} 
% \vspace{1cm}
% Sincerely yours, \\
% \vspace{1cm}
% Jingzhi Gong

% \end{flushleft} 






